HeadText: Exploring Hands-free Text Entry using Head Gestures by Motion Sensing on a Smart Earpiece

We present HeadText, a hands-free technique on a smart earpiece for text entry by motion sensing. Users input text utilizing only 7 head gestures for key selection, word selection, word commitment and word cancelling tasks. Head gesture recognition is supported by motion sensing on a smart earpiece to capture head moving signals and machine learning algorithms (K-Nearest-Neighbor (KNN) with a Dynamic Time Warping (DTW) distance measurement). A 10-participant user study proved that HeadText could recognize 7 head gestures at an accuracy of 94.29%. After that, the second user study presented that HeadText could achieve a maximum accuracy of 10.65 WPM and an average accuracy of 9.84 WPM for text entry. Finally, we demonstrate potential applications of HeadText in hands-free scenarios for (a). text entry of people with motor impairments, (b). private text entry, and (c). socially acceptable text entry.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.75.  \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.76.  Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.77.  Changed the way to typset multiple affiliations (Christoph Sommer)

==> ncctools/source/README <==
README for the `ncctools' bundle
================================

This `bundle' consists of LaTeX2e packages written and supported by
Alexander I. Rozhenko.

The documented source code of all packages is in files with extension
`.dtx'.  To install the bungle, run

  latex ncctools.ins

It will produce the package files from all `.dtx' files.
The files with extensions `.sty' should then be moved to a directory
on LaTeX's standard input path.

License Agreement
=================

This material is subject to the LaTeX Project Public License.
See http://www.ctan.org/tex-archive/help/Catalogue/licenses.lppl.html
for the details of that license.

NOTE (docstrip version)
***********************
****
**** If   latex ncctools.ins
**** produces the `docstrip interactive mode' prompt:
****
****   * First type the extension of your input file(s):  *
****   \infileext=
****
**** Then your version of docstrip is too old.
**** Quit (eg by hitting `enter' to all questions) and get a newer
**** docstrip.tex. It must be at least version 2.4.
****
**** A suitable docstrip.tex may be found from `CTAN' archives such as
**** ftp.dante.de   tex-archive/macros/latex/unpacked/docstrip.tex
****
**** Docstrip is part of the base LaTeX distribution, so if you have
**** an old docstrip then your LaTeX is out of date and you may consider
**** getting the whole of that directory and re-installing LaTeX.
**** However you need to fetch only the file docstrip.tex to unpack
**** this tools distribution with your existing format.


Documentation for the individual documented packages may then be
obtained by running LaTeX on the `.dtx' files.

For example:

  latex manyfoot.dtx

will produce the file manyfoot.dvi, documenting the manyfoot package.

***NOTE****
Copyright is maintained by Alexander I. Rozhenko.

All the packages in this bundle are released under the restrictions
detailed below.

The file manifest.txt contains a list of files in the distribution.


Reporting Bugs
==============

To report a problem or bug in any of these packages, describe it in free
form and send it me to e-mail address

        rozhenko@oapmg.sscc.ru

Type the `NCCTOOLS' word in the subject of letter. This guarantees
that your letter will be not deleted as spam.

When reporting bugs, please produce a small test file that shows the
problem, and ensure that you are using the current version of the
package, and of the base LaTeX software.


Distribution of unchanged versions
==================================

  Redistribution of unchanged files is allowed provided that this
  readme file is included and all the files for a package are
  distributed together.

Generation and distribution of changed versions
===============================================

  The generation of changed versions of the files included in these
  packages is allowed under the restrictions listed in the file
  legal.txt in the base LaTeX distribution.  In particular you should:

  - rename the file before you make any changes to it.

  - change the error report address so that I do not get sent error
    reports for files *not* maintained by me.

  The distribution of changed versions of the files included in these
  packages is allowed under the restrictions listed in the file
  legal.txt in the base LaTeX distribution.  In particular you should:

  - also distribute the unmodified version of the file.


==> xstring.tex <==
% !TeX encoding = ISO-8859-1
% Ce fichier contient le code de l'extension "xstring"
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                                    %
\def\xstringname               {xstring}                             %
\def\xstringversion              {1.83}                              %
%                                                                    %
\def\xstringdate              {2019/02/06}                           %
%                                                                    %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                                    %
% Author     : Christian Tellechea                                   %
% Status     : Maintained                                            %
% Maintainer : Christian Tellechea                                   %
% Email      : unbonpetit@netc.fr                                    %
% Package URL: https://www.ctan.org/pkg/xstring                      %
% Bug tracker: https://framagit.org/unbonpetit/xstring/issues        %
% Repository : https://framagit.org/unbonpetit/xstring/tree/master   %
% Copyright  : Christian Tellechea 2008-2019                         %
% Licence    : Released under the LaTeX Project Public License v1.3c %
%              or later, see http://www.latex-project.org/lppl.txt   %
% Files      : 1) xstring.tex                                        %
%              2) xstring.sty                                        %
%              3) xstring-fr.tex                                     %
%              4) xstring-fr.pdf                                     %
%              5) xstring-en.tex                                     %
%              6) xstring-en.pdf                                     %
%              7) README                                             %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\ifdefined\usepackage\else
	\immediate\write-1 {Package: xstring \xstringdate\space v\xstringversion\space String manipulations (CT)}%
\fi
\newcount\integerpart
\newcount\decimalpart% compteurs utilisés par xstring

\edef\restorexstringcatcode{\catcode\number`\_ =\number\catcode`\_\relax}
\catcode`\_=11

\long\def\xs_execfirst#1#2{#1}
\long\def\xs_execsecond#1#2{#2}
\long\def\xs_gobarg#1{}
\expandafter\def\expandafter\xs_gobspace\space{}
\def\xs_deftok#1#2{\let#1= #2\relax}\xs_deftok\xs_sptoken{ }
\long\def\xs_ifnxttok#1#2#3{\xs_deftok\xs_toksmatch{#1}\def\__truecode{#2}\def\__falsecode{#3}\xs_ifnxttok_a}
\def\xs_ifnxttok_a{\futurelet\__futurtok\xs_ifnxttok_b}
\def\xs_ifnxttok_b{%
	\xs_ifx{\__futurtok\xs_sptoken}
		{\afterassignment\xs_ifnxttok_a\let\__futurtok= }
		{\xs_ifx{\__futurtok\xs_toksmatch}\__truecode\__falsecode}%
}
\def\xs_ifstar#1{\xs_ifnxttok*{\xs_execfirst{#1}}}
\long\def\xs_testopt#1#2{\xs_ifnxttok[{#1}{#1[{#2}]}}
\long\def\xs_exparg#1#2{\expandafter\xs_exparg_a\expandafter{#2}{#1}}%
\long\def\xs_exparg_a#1#2{#2{#1}}
\long\def\xs_exptwoargs#1#2#3{\xs_exparg{\xs_exparg{#1}{#2}}{#3}}
\long\def\xs_eearg#1#2{\xs_exparg{\xs_exparg{#1}}{#2}}
\long\def\xs_edefaddtomacro#1#2{\edef#1{\unexpanded\expandafter{#1}#2}}
\long\def\xs_addtomacro#1#2{\xs_exparg{\def#1}{#1#2}}
\long\def\xs_eaddtomacro#1#2{\xs_exparg{\xs_addtomacro#1}{#2}}
\long\def\xs_eeaddtomacro#1#2{\xs_exparg{\xs_eaddtomacro#1}{#2}}
\long\def\xs_endgroup_eaddtomacro#1#2{\xs_exparg{\endgroup\xs_addtomacro#1}{#2}}
\long\def\xs_beforespace#1 #2\_nil{#1}
\long\def\xs_afterspace#1 #2\_nil{#2}
\long\def\xs_gobtonil#1\_nil{}
\long\def\xs_gobtobrace#1#{}
\long\def\xs_ifx#1{\ifx#1\expandafter\xs_execfirst\else\expandafter\xs_execsecond\fi}
\def\xs_ifnum#1{\ifnum#1\expandafter\xs_execfirst\else\expandafter\xs_execsecond\fi}
\long\def\xs_ifempty#1{\expandafter\xs_ifx\expandafter{\expandafter\relax\detokenize{#1}\relax}}

\def\xs_toks_toverb{% lit 1 argument et le transforme en verb
	\begingroup
		\def\do##1{\catcode`##112 }%
		\dospecials
		\obeyspaces
		\xs_read_verb
}

\def\setverbdelim#1{% définit quel est le délimiteur de verb
	\xs_exparg\xs_ifempty{\xs_gobarg#1}%
		{}
		{\errmessage{Package xstring Warning: verb delimiter "\detokenize{#1}" is not a single token}}%
	\def\xs_read_verb##1#1##2#1{\endgroup\xs_assign_verb{##2}}% on appelle l'exécution de fin
}

% Assigne l'argument entre délimiteur verb dans la sc #1
\def\verbtocs#1{%
	\def\xs_assign_verb##1{\def#1{##1}}%
	\xs_toks_toverb
}

\begingroup
	\catcode0 3 \gdef\xs_twozeroschars{^^00}%
	\catcode0 7 \xdef\xs_twozeroschars{\xs_twozeroschars^^00}%
\endgroup

\edef\xs_reserved_A{\long\def\noexpand\xs_assigntokenizeresult##1\xs_twozeroschars}
\xs_reserved_A#2{\endgroup\xs_exparg{\def#2}{\xs_gobarg#1}}

\def\tokenize#1#2{%
	\begingroup
		\xs_def\xs_reserved_A{#2}% on développe en accord avec \fullexpandarg ou \noexpandarg
		\everyeof\expandafter{\xs_twozeroschars#1}%
		\endlinechar-1
		\expandafter\xs_assigntokenizeresult\scantokens\expandafter{\expandafter\relax\xs_reserved_A}% on fait l'assignation
}%

\long\def\xs_assign_xstringresult#1#2{\xs_ifempty{#2}{#1}{\def#2{#1}}}

\def\xs_ldef{\long\def}
\def\xs_ledef{\long\edef}

\def\normalexpandarg{%
	\let\xs_def\xs_ldef% on définit \xs_call avec \def
	\def\xs_expand##1{\unexpanded\expandafter{##1}}%
}
\let\noexpandarg\normalexpandarg% synonyme

\def\expandarg{%
	\let\xs_def\xs_ldef% on définit \xs_call avec \def
	\def\xs_expand##1{\unexpanded\expandafter\expandafter\expandafter{##1}}%
}

\def\fullexpandarg{%
	\let\xs_def\xs_ledef% on définit\xs_call avec \edef
	\def\xs_expand##1{##1}% et on neutralise \xs_expand
}

\def\saveexpandmode{\let\xs_saved_def\xs_defarg\let\xs_saved_expand\xs_expand}
\def\restoreexpandmode{\let\xs_defarg\xs_saved_def\let\xs_expand\xs_saved_expand}

% Macro interne renvoyant #2 si son argument commence par une accolade ouvrante "{"
% et #3 sinon (Ulrich Diez sur comp.text.tex)
\long\def\xs_ifbeginwithbrace#1{%
	\csname xs_exec%
		\expandafter\xs_gobarg\string{%
		\expandafter\xs_gobarg\expandafter{\expandafter{\string#1}%
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\xs_execfirst
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\xs_gobarg
		\expandafter\expandafter\expandafter\xs_gobarg
		\expandafter\expandafter\expandafter{\expandafter\string\expandafter}\string}%
		\expandafter\xs_gobarg\string}%
		\xs_execsecond{first}{second}%
	\endcsname
}

% Cette macro interne prend la 1ere unité syntaxique de #1 et assigne le résultat à #2
\long\def\xs_returnfirstsyntaxunit#1#2{%
	\let\xs_toks\relax
	\xs_ifempty{#1}
		{\let#2\empty
		}
		{\xs_eearg\xs_ifempty{\expandafter\xs_beforespace\detokenize{#1} \_nil}% #1 commence par un espace ?
			{\def#2{ }}
			{\xs_ifbeginwithbrace{#1}
				{\def\xs_groupfound{\xs_exparg{\def#2}{\expandafter{#2}}\xs_gobtonil}% on met #2 dans des accolades et on finit
				\let\xs_toks\bgroup
				\afterassignment\xs_groupfound
				\def#2%
				}
				{\long\def\xs_assignfirstarg##1##2\_nil{\def#2{##1}}%
				\xs_assignfirstarg
				}%
			#1\_nil
			}%
		}%
}

\long\def\xs_removefirstsyntaxunit#1#2{%
	\xs_ifempty{#1}
		{\let#2\empty
		}
		{\xs_eearg\xs_ifempty{\expandafter\xs_beforespace\detokenize{#1} \_nil}% #1 commence par un espace ?
			{\xs_exparg\xs_ifbeginwithbrace{\xs_gobspace#1}
				{\xs_exparg{\def#2}{\xs_gobtobrace#1}}%
				{\xs_exparg{\def#2}{\xs_afterspace#1\_nil}}%
			}%
			{\xs_exparg{\def#2}{\xs_gobarg#1}}%
		}%
}

% Cette macro interne est utilisée dans les macros étoilées pour :
% 1) développer l'argument selon qu'on a choisit \fullexpandarg
%    ou \normalexpandarg, et ceci à l'aide de la macro \xs_def
% 2) Ensuite, on détokenize ce développement de façon n'avoir plus que
%    des catcodes de 10 pour les espaces et 12 pour le reste.
\long\def\xs_expand_and_detokenize#1#2{%
	\long\def#1{#2}%
	\expandafter\edef\expandafter#1\expandafter{\xs_expand#1}% on développe #2 selon le mode de développement
	\long\edef#1{\detokenize\expandafter{#1}}% puis on détokenize et on assigne à #1
}

\long\def\xs_expand_and_assign#1#2{\xs_def#1{#2}}% on développe #2 selon \fullexpandarg ou \normalexpandarg

\def\xs_arglist{0########1########2########3########4########5########6########7########8########9}

% \xs_assign_args{3} met dans la sc \xs_myarg les tokens "####1####2####3"
\def\xs_assign_args#1{\def\xs_assign_args_i0##1#1##2\_nil{\def\xs_myarg{##1#1}}\expandafter\xs_assign_args_i\xs_arglist\_nil}

% \xs_assign_opt_args{3} met dans la sc \xs_myarg les tokens "[####1]####2####3####4"
\def\xs_assign_opt_args#1{\xs_exparg\xs_assign_opt_args_i{\number\numexpr#1+1}}
\def\xs_assign_opt_args_i#1{\def\xs_assign_opt_args_ii0##11##2#1##3\_nil{\def\xs_myarg{[##11]##2#1}}\expandafter\xs_assign_opt_args_ii\xs_arglist\_nil}

% \xs_assign_one_arg{3} met dans la sc \xs_myarg les tokens "####3"
\def\xs_assign_one_arg#1{\xs_exparg\xs_assign_one_arg_i{\number\numexpr#1-1}{#1}}
\def\xs_assign_one_arg_i#1#2{\def\xs_assign_one_arg_ii##1#1##2#2##3\_nil{\def\xs_myarg{##2#2}}\expandafter\xs_assign_one_arg_ii\xs_arglist\_nil}

% #1 : numéro du 1er argument; #2 : nombre de lignes; #3 argument optionnel; #4 : dernier numéro de l'argument devant être détokenisé si étoile
\def\xs_buildlines#1#2#3#4{%
	\let\xs_newlines\empty
	\let\xs_newargs\empty
	\def\xs_buildlines_i##1{%
		\xs_exparg\xs_assign_one_arg{\number\numexpr##1+#1-1}%
		\edef\xs_reserved_B{\noexpand\xs_expand\csname xs_arg_\romannumeral\numexpr##1\endcsname}%
		\xs_ifnum{##1=1 }% si c'est le premier argument
			{\xs_ifempty{#3}%
				{\xs_eaddtomacro\xs_newargs{\expandafter{\xs_reserved_B}}%
				\edef\xs_reserved_B{\ifnum##1>#4 xs_def\else xs_assign\fi}%
				}% et s'il y a un argument optionnel alors, on met des crochets
				{\xs_eaddtomacro\xs_newargs{\expandafter[\xs_reserved_B]}%
				\def\xs_reserved_B{xs_def}% ne pas détokéniser l'argument optionnel grace au \xs_def
				}%
			}
			{\xs_eaddtomacro\xs_newargs{\expandafter{\xs_reserved_B}}%
			\edef\xs_reserved_B{\ifnum##1>#4 xs_def\else xs_assign\fi}%
			}%
		\edef\xs_newlines{\unexpanded\expandafter{\xs_newlines}\expandafter\noexpand\csname\xs_reserved_B\endcsname\expandafter\noexpand\csname xs_arg_\romannumeral\numexpr##1\endcsname{\xs_myarg}}%
		\xs_ifnum{##1<#2 }
			{\xs_exparg\xs_buildlines_i{\number\numexpr##1+1}}
			{}%
	}%
	\xs_buildlines_i1%
}

\def\xs_newmacro{%
	\xs_ifstar
		{\let\xs_reserved_D\empty\xs_newmacro_}
		{\let\xs_reserved_D\relax\xs_newmacro_0}%
}

% #1 : dernier numéro de l'argument devant être détokenisé
% #2 : nom de la macro publique
% #3 : argument optionnel (vide si pas d'arg optionnel)
% #4 : nombre d'arguments obligatoires
% #5 : utilisation de testopt (1 si oui, 0 si non)
% #6 : code de la macro
\def\xs_newmacro_#1#2#3#4#5{%
	\edef\xs_reserved_A{xs_\expandafter\xs_gobarg\string#2}%
	\edef\xs_reserved_C{\expandafter\noexpand\csname\xs_reserved_A _\ifx\empty#3\empty _\fi\endcsname}%
	\edef\xs_reserved_B{%
		\long
		\ifx\empty\xs_reserved_D
			\def\noexpand#2{\noexpand\xs_ifstar
				{\let\noexpand\xs_assign\noexpand\xs_expand_and_detokenize\expandafter\noexpand\xs_reserved_C}%
				{\let\noexpand\xs_assign\noexpand\xs_expand_and_assign\expandafter\noexpand\xs_reserved_C}%
			}%
		\else
			\def\noexpand#2{\let\noexpand\xs_assign\noexpand\xs_expand_and_assign\expandafter\noexpand\xs_reserved_C}%
		\fi
		\ifx\empty#3\empty
		\else
			\def\expandafter\noexpand\xs_reserved_C{%
				\noexpand\xs_testopt{\expandafter\noexpand\csname\xs_reserved_A __\endcsname}{\ifx\xs_def\xs_ledef#3\else\unexpanded{#3}\fi}}%
		\fi
	}%
	% Que fait \xs_reserved_B ? Il définit :
	% si #3 est vide : \NOM{\xs_ifstar{\let\xs_assign\xs_expand_and_detokenize\xs_NOM__}{\let\xs_assign\xs_expand_and_assign\xs_NOM__}}
	% si #3 existe   : \NOM{\xs_ifstar{\let\xs_assign\xs_expand_and_detokenize\xs_NOM_}{\let\xs_assign\xs_expand_and_assign\xs_NOM_}}
	%                  \xs_NOM_{\xs_testopt{\xs_NOM__}{#3}}}
	\xs_reserved_B
	\ifx\empty#3\empty
		\xs_buildlines1{#4}{#3}{#1}%
		\xs_assign_args{#4}%
	\else
		\xs_exparg{\xs_buildlines1}{\number\numexpr#4+1}{#3}{#1}%
		\xs_assign_opt_args{#4}%
	\fi
	\edef\xs_reserved_B{\def\expandafter\noexpand\csname\xs_reserved_A __\endcsname\xs_myarg}%
	\edef\xs_reserved_C{\unexpanded\expandafter{\xs_newlines}\edef\noexpand\xs_call}%
	\edef\xs_reserved_D{\noexpand\noexpand\expandafter\noexpand\csname\xs_reserved_A\endcsname\unexpanded\expandafter{\xs_newargs}}%
	\ifnum#5=1 \edef\xs_reserved_D{\noexpand\noexpand\noexpand\xs_testopt{\unexpanded\expandafter{\xs_reserved_D}}{}}\fi
	\xs_edefaddtomacro\xs_reserved_C{{\unexpanded\expandafter{\xs_reserved_D}}\noexpand\xs_call}%
	\xs_edefaddtomacro\xs_reserved_B{{\unexpanded\expandafter{\xs_reserved_C}}}%
	% Que fait \xs_reserved_B ? Il définit par exemple pour 3 arguments obligatoires et 1 facultatif :
	%    \def\xs_NOM__[##2]##3##4##5{%
	%          \xs_def\xs_arg_i{##2}\xs_assign\xs_arg_ii{##3}\xs_assign\xs_arg_iii{##4}\xs_asign\xs_arg_iv{##5}%
	% si #5=0: \edef\xs_call{\noexpand\xs_NOM[\xs_expand\xs_arg_i]{\xs_expand\xs_arg_ii}{\xs_expand\xs_arg_iii}{\xs_expand\xs_arg_iv}}%
	% si #5=1: \edef\xs_call{\noexpand\xs_testopt{\noexpand\xs_NOM[\xs_expand\xs_arg_i]{\xs_expand\xs_arg_i}{\xs_expand\xs_arg_ii}{\xs_expand\xs_arg_iii}{\xs_expand\xs_arg_iv}}{}}%
	%          \xs_call}
	\long\xs_reserved_B
	\edef\xs_reserved_B{%
		\def\expandafter\noexpand\csname\xs_reserved_A\endcsname
			\xs_myarg\ifnum#5=1 [\unexpanded{##}\number\numexpr\ifx\empty#3\empty#4+1\else#4+2\fi]\fi
	}%
	% Que fait \xs_reserved_B ? Il définit par exemple pour 3 arguments obligatoires et 1 facultatif :
	%    \def \xs_NOM[##2]##3##4##5[##6]{#6}
	\long\xs_reserved_B
}

% macro générique qui lit \xs_reserved_C us par us
% 3 sous-routines sont appelées à des moments clé :
% \xs_atendofgroup      (un groupe se finit, appel récursif)
% \xs_atbegingroup      (un groupe vient d'être ouvert)
% \xs_atnextsyntaxunit  (la future US n'est pas un groupe)
\def\xs_read_reserved_C{%
	\xs_exparg\xs_ifempty{\xs_reserved_C}%
		{\xs_ifnum{\xs_nestlevel=0 }
			{}
			{\xs_atendofgroup
			\xs_read_reserved_C
			}%
		}
		{\xs_exparg\xs_returnfirstsyntaxunit{\xs_reserved_C}\xs_reserved_A
		\xs_exparg\xs_removefirstsyntaxunit{\xs_reserved_C}\xs_reserved_C
		\xs_exploregroups
		\xs_ifx{\bgroup\xs_toks}
			{\advance\integerpart1
			\begingroup
				\expandafter\def\expandafter\xs_reserved_C\xs_reserved_A
				\xs_calc_grouIP
				\def\xs_nestlevel{1}%
				\integerpart0
				\xs_atbegingroup
			}
			{\advance\decimalpart1
			\xs_atnextsyntaxunit
			}%
		\xs_read_reserved_C
		}%
}

% macro générique qui lit \xs_reserved_D en procédant à des tests avec \IfBeginWith
% 1 sous-routine est appelée :
% \xs_atoccurfound      (une occurrence a été trouvée)
\def\xs_read_reserved_D{%
	\xs_exparg\xs_ifempty{\xs_reserved_D}%
		{\xs_ifnum{\xs_nestlevel=0 }
			{}
			{\edef\__temp{%
				\endgroup
				\noexpand\decimalpart=\number\decimalpart\relax
				\unexpanded{\xs_addtomacro\xs_reserved_C}{{\unexpanded\expandafter{\xs_reserved_C}}}%
				}%
			\__temp
			\xs_read_reserved_D
			}%
		}%
		{\xs_exptwoargs\xs_IfBeginWith_i\xs_reserved_D\xs_reserved_E
			{\advance\decimalpart1
			\let\xs_reserved_D\xs_reserved_A
			\xs_atoccurfound
			}%
			{\xs_exparg\xs_returnfirstsyntaxunit{\xs_reserved_D}\xs_reserved_A
			\xs_exparg\xs_removefirstsyntaxunit{\xs_reserved_D}\xs_reserved_D
			\xs_exploregroups
			\xs_ifx{\bgroup\xs_toks}
				{\advance\integerpart1
				\begingroup
					\expandafter\def\expandafter\xs_reserved_D\xs_reserved_A
					\xs_calc_grouIP
					\let\xs_reserved_C\empty
					\def\xs_nestlevel{1}%
					\integerpart0
				}
				{\xs_eaddtomacro\xs_reserved_C{\xs_reserved_A}%
				}%
			}%
		\xs_read_reserved_D
		}%
}

\xs_newmacro\StrRemoveBraces{}{1}{1}{%
	\def\xs_reserved_C{#1}%
	\let\xs_reserved_B\empty
	\def\xs_nestlevel{0}%
	\xs_StrRemoveBraces_i
	\xs_exparg\xs_assign_xstringresult{\xs_reserved_B}{#2}%
}

\def\xs_StrRemoveBraces_i{%
	\xs_exparg\xs_ifempty{\xs_reserved_C}%
		{\xs_ifnum{\xs_nestlevel=0 }
			{}
			{\xs_endgroup_eaddtomacro\xs_reserved_B\xs_reserved_B
			\xs_StrRemoveBraces_i
			}%
		}
		{\xs_exparg\xs_returnfirstsyntaxunit{\xs_reserved_C}\xs_reserved_A
		\xs_exparg\xs_removefirstsyntaxunit{\xs_reserved_C}\xs_reserved_C
		\xs_ifx{\bgroup\xs_toks}
			{\xs_ifx{\xs_exploregroups\relax}% on explore les groupes ?
				{\begingroup
					\expandafter\def\expandafter\xs_reserved_C\xs_reserved_A
					\def\xs_nestlevel{1}%
					\let\xs_reserved_B\empty
				}
				{\expandafter\xs_addtomacro\expandafter\xs_reserved_B\xs_reserved_A
				}%
			}
			{\xs_eaddtomacro\xs_reserved_B{\xs_reserved_A}%
			}%
		\xs_StrRemoveBraces_i
		}%
}

% \xs_cutafteroccur coupe l'argument #1 après la #3ème occurrence de #2
% \xs_reserved_C : contient ce qui se trouve avant cette occurrence
% \xs_reserved_D : contient ce qui se trouve avant cette occurrence y compris cette occurrence
% \xs_reserved_E : contient ce qui se trouve après l'occurrence
% si l'occurrence n'existe pas ou qu'un des arguments est vide, toutes les chaines renvoyées sont vides
\long\def\xs_cutafteroccur#1#2#3{%
	\xs_ifnum{#3<1 }
		{\let\xs_reserved_C\empty\let\xs_reserved_E\empty\gdef\groupID{}}
		{\xs_cutafteroccur_i{#1}{#2}{#3}}%
}
	
\long\def\xs_cutafteroccur_i#1#2#3{%
	\def\xs_reserved_D{#1}\let\xs_reserved_C\empty\def\xs_reserved_E{#2}%
	\decimalpart0 \integerpart0 \gdef\groupID{0}\def\xs_nestlevel{0}%
	\def\xs_atoccurfound{%
		\xs_ifnum{\decimalpart=\numexpr(#3)\relax}
			{\edef\__temp{%
				\def\noexpand\xs_reserved_C{\unexpanded\expandafter{\xs_reserved_C}}%
				\def\noexpand\xs_reserved_D{\unexpanded\expandafter{\xs_reserved_D}}%
				\noexpand\decimalpart=\number\decimalpart\relax
				}%
			\expandafter\xs_exitallgroups\__temp
			\xs_gobarg% mange l'appel récursif \xs_read_reserved_D dans \xs_read_reserved_D
			}
			{\xs_eaddtomacro\xs_reserved_C{\xs_reserved_E}%
			}%
	}%
	\xs_read_reserved_D
	\xs_ifnum{\decimalpart=\numexpr(#3)\relax}% occurrence trouvée ?
		{\let\xs_reserved_E\xs_reserved_D
		\xs_exparg{\def\xs_reserved_D}{\xs_reserved_C#2}%
		}
		{\let\xs_reserved_C\empty
		\let\xs_reserved_E\empty
		\gdef\groupID{}%
		}%
}

\xs_newmacro*3\IfSubStr{1}{2}{0}{%
	\xs_cutafteroccur{#2}{#3}{#1}%
	\xs_exparg\xs_ifempty{\xs_reserved_D}\xs_execsecond\xs_execfirst
}

\xs_newmacro*2\IfBeginWith{}{2}{0}{%
	\xs_ifempty{#2}%
		{\xs_execsecond}
		{\xs_IfBeginWith_i{#1}{#2}}%
}

\long\def\xs_IfBeginWith_i#1#2{%
	\xs_ifempty{#2}%
		{\xs_execfirst% #2 est vide, tous les tests sont passés avec succès : on renvoie #3
		}
		{\xs_ifempty{#1}%
			{\xs_execsecond% #1 est vide, c'est que #2 est + long que #1 : on renvoie #4
			}
			{\xs_returnfirstsyntaxunit{#2}\xs_reserved_B
			\xs_returnfirstsyntaxunit{#1}\xs_reserved_A
			\xs_ifx{\xs_reserved_A\xs_reserved_B}% il y a égalité...
				{\xs_removefirstsyntaxunit{#2}\xs_reserved_B
				\xs_removefirstsyntaxunit{#1}\xs_reserved_A% on enlève les 1ere unités syntaxiques
				\xs_exptwoargs\xs_IfBeginWith_i\xs_reserved_A\xs_reserved_B
				}
				{\xs_execsecond
				}%
			}%
		}%
}

\xs_newmacro*2\IfEndWith{}{2}{0}{%
	\xs_ifempty{#2}%
		{\xs_execsecond
		}
		{\xs_StrCount{#1}{#2}[\xs_reserved_A]%
		\xs_ifnum{\xs_reserved_A=0 }
			{\xs_execsecond}
			{\xs_exparg\xs_ifempty{\xs_reserved_C}}%
		}%
}

\xs_newmacro*4\IfSubStrBefore{1,1}{3}{0}{\xs_IfSubStrBefore_i[#1]{#2}{#3}{#4}}

\def\xs_IfSubStrBefore_i[#1,#2]#3#4#5{%
	\def\xs_reserved_C{#3}%
	\xs_ifx{\xs_exploregroups\relax}% si on explore les groupes
		{\let\xs_reserved_B\empty
		\def\xs_nestlevel{0}%
		\xs_StrRemoveBraces_i% on retire les accolades
		\let\xs_reserved_C\xs_reserved_B
		}
		{}%
	\xs_exparg\xs_cutafteroccur\xs_reserved_C{#5}{#2}%
	\xs_exparg\xs_cutafteroccur\xs_reserved_C{#4}{#1}%
	\gdef\groupID{}%
	\xs_exparg\xs_ifempty{\xs_reserved_C}%
		\xs_execsecond
		\xs_execfirst
}

\xs_newmacro*4\IfSubStrBehind{1,1}{3}{0}{\xs_IfSubStrBehind_i[#1]{#2}{#3}{#4}}
\long\def\xs_IfSubStrBehind_i[#1,#2]#3#4#5{\xs_IfSubStrBefore_i[#2,#1]{#3}{#5}{#4}}

\long\def\xs_formatnumber#1#2{%
	\xs_ifempty{#1}%
		{\def#2{0X}% si vide, renvoie 0X
		}
		{\xs_returnfirstsyntaxunit{#1}\xs_reserved_A
		\def\xs_reserved_B{+}%
		\xs_ifx{\xs_reserved_A\xs_reserved_B}
			{\xs_removefirstsyntaxunit{#1}\xs_reserved_C
			\xs_exparg\xs_ifempty{\xs_reserved_C}%
				{\def#2{+0X}}
				{\xs_exparg{\def#2}{\expandafter+\expandafter0\xs_reserved_C}}%
			}
			{\def\xs_reserved_B{-}%
			\xs_ifx{\xs_reserved_A\xs_reserved_B}
				{\xs_removefirstsyntaxunit{#1}\xs_reserved_A
				\xs_exparg\xs_ifempty{\xs_reserved_A}%
					{\def#2{-0X}}%
					{\xs_exparg{\def#2}{\expandafter-\expandafter0\xs_reserved_A}}%
				}
				{\def#2{0#1}%
				}%
			}%
		}%
}

\xs_newmacro\IfInteger{}{1}{0}{%
	\xs_formatnumber{#1}\xs_reserved_A
	\decimalpart0
	\afterassignment\xs_defafterinteger\integerpart\xs_reserved_A\relax\_nil
	\let\xs_after_intpart\afterinteger
	\expandafter\xs_testdot\afterinteger\_nil
	\xs_ifx{\empty\afterdecimal}
		{\xs_ifnum{\decimalpart=0 }
			{\xs_execfirst% partie décimale constituée de 0 --> seul cas où on renvoie vrai
			}
			{\expandafter\xs_defafterinteger\xs_after_intpart\relax\_nil
			\xs_execsecond
			}%
		}
		{\expandafter\xs_defafterinteger\xs_after_intpart\relax\_nil
		\xs_execsecond
		}%
}

\xs_newmacro\IfDecimal{}{1}{0}{%
	\xs_formatnumber{#1}\xs_reserved_A
	\decimalpart0
	\afterassignment\xs_defafterinteger\integerpart\xs_reserved_A\relax\_nil
	\expandafter\xs_testdot\afterinteger\_nil
	\xs_ifx{\empty\afterdecimal}
}

\begingroup\catcode`\@ 11
\long\gdef\xs_defafterinteger#1\relax\_nil{\def\@xs@afterinteger{#1}\let\afterinteger\@xs@afterinteger}
\long\gdef\xs_defafterdecimal#1\_nil{\def\@xs@afterdecimal{#1}\let\afterdecimal\@xs@afterinteger}
\endgroup

\def\xs_testdot{%
	\let\xs_decsep\empty
	\xs_ifnxttok.
		{\def\xs_decsep{.}\xs_readdecimalpart}%
		{\xs_testcomma}%
}

\def\xs_testcomma{%
	\xs_ifnxttok,
		{\def\xs_dessep{,}\xs_readdecimalpart}%
		{\xs_defafterdecimal}%
}

\long\def\xs_readdecimalpart#1#2\_nil{%
	\xs_ifempty{#2}
		{\def\xs_reserved_A{0X}}
		{\def\xs_reserved_A{0#2}}%
	\afterassignment\xs_defafterinteger\decimalpart\xs_reserved_A\relax\_nil
	\expandafter\xs_defafterdecimal\afterinteger\_nil
}

% test d'égalité sur des chaines (et des chaines contenant des nombres)
\long\def\xs_IfStrEqFalse_i#1#2{\let\xs_reserved_A\xs_execsecond}
\long\def\xs_IfStrEqFalse_ii#1#2{% renvoie vrai si les 2 arg sont décimaux et s'ils sont égaux, faux sinon
	\xs_IfDecimal{#1}%
		{\xs_IfDecimal{#2}%
			{\ifdim#1pt=#2pt
				\let\xs_reserved_A\xs_execfirst
			\else
				\let\xs_reserved_A\xs_execsecond
			\fi% les 2 sont décimaux : on fait le test
			}%
			{\let\xs_reserved_A\xs_execsecond}% un seul est décimal
		}%
		{\let\xs_reserved_A\xs_execsecond}% #1 n'est pas décimal
}

\long\def\xs_TestEqual#1#2{% teste si les 2 arguments sont égaux
	\def\xs_reserved_A{#1}\def\xs_reserved_B{#2}%
	\xs_ifx{\xs_reserved_A\xs_reserved_B}
		{\let\xs_reserved_A\xs_execfirst}% égalité parfaite des 2 chaines
		{\xs_reserved_D{#1}{#2}}%
	\xs_reserved_A
}

\xs_newmacro*2\IfStrEq{}{2}{0}{% teste si les deux chaines sont égales
	\let\xs_reserved_D\xs_IfStrEqFalse_i
	\xs_TestEqual{#1}{#2}%
}

\xs_newmacro*2\IfEq{}{2}{0}{% teste si les 2 arguments (chaine ou nombre) sont égaux
	\let\xs_reserved_D\xs_IfStrEqFalse_ii
	\xs_TestEqual{#1}{#2}%
}

\def\IfStrEqCase{%
	\xs_ifstar
		{\xs_IfStringCase{\IfStrEq*}}%
		{\xs_IfStringCase\IfStrEq}%
}

\def\IfEqCase{%
	\xs_ifstar
		{\xs_IfStringCase{\IfEq*}}%
		{\xs_IfStringCase\IfEq}%
}

\long\def\xs_IfStringCase#1#2#3{% #1=macro avec ou sans étoile  #2=argument à tester  #3=liste des {<cas>}{code>}
	\long\def\xs_testcase##1##2##3\_nil{% lit les 2 premieres unités syntaxiques dans ##1 et ##2. Les autres dans ##3
		#1{#2}{##1}% compare
			{\xs_testopt{\xs_IfStringCase_ii{##2}}{}}% le test est positif, on exécute le code correspondant et on mange l'argument optionnel ## BUGfix dans 1.82
			{\xs_ifempty{##3}%
				{\xs_testopt{\xs_IfStringCase_i}{}}% s'il n'y a plus de cas, on exécute le code <autres cas> ## BUGfix dans 1.82
				{\xs_testcase##3\_nil}% sinon, on recommence avec ce qui reste
			}%
	}%
	\xs_testcase#3\_nil
}

\long\def\xs_IfStringCase_i[#1]{#1}
\long\def\xs_IfStringCase_ii#1[#2]{#1}

% Renvoie ce qui est à gauche de l'occurence n°#1 de la sous chaine #3 dans la chaine #2
\xs_newmacro*3\StrBefore{1}{2}{1}{%
	\xs_cutafteroccur{#2}{#3}{#1}%
	\xs_exparg\xs_assign_xstringresult{\xs_reserved_C}{#4}%
}

% Renvoie ce qui est à droite de l'occurence n°#1 de la sous chaine #3 dans la chaine #2
\xs_newmacro*3\StrBehind{1}{2}{1}{%
	\xs_cutafteroccur{#2}{#3}{#1}%
	\xs_exparg\xs_assign_xstringresult{\xs_reserved_E}{#4}%
}

% Renvoie ce qui est strictement compris entre les occurrences n°#1 et n°#2
% des chaines #4 et #5 dans la chaine #3
\xs_newmacro*4\StrBetween{1,1}{3}{1}{\xs_StrBetween_i[#1]{#2}{#3}{#4}[#5]}
\long\def\xs_StrBetween_i[#1,#2]#3#4#5[#6]{%
	\begingroup
		\noexploregroups
		\xs_cutafteroccur{#3}{#5}{#2}%
		\xs_exparg\xs_cutafteroccur{\xs_reserved_C}{#4}{#1}%
		\expandafter
	\endgroup
	\expandafter\xs_assign_xstringresult\expandafter{\xs_reserved_E}{#6}%
	\gdef\groupID{}%
}

\def\exploregroups{\let\xs_exploregroups\relax}
\def\noexploregroups{\def\xs_exploregroups{\let\xs_toks\relax}}
\def\saveexploremode{\let\xs_saveexploremode\xs_exploregroups}
\def\restoreexploremode{\let\xs_exploregroups\xs_saveexploremode}

% Remplace les #1 premières occurences de la chaine #3
% par la chaine #4 dans la chaine #2
\xs_newmacro\StrSubstitute{0}{3}{1}{%
	\def\xs_reserved_D{#2}\let\xs_reserved_C\empty\def\xs_reserved_E{#3}%
	\decimalpart0 \integerpart0 \gdef\groupID{0}\def\xs_nestlevel{0}%
	\def\xs_atoccurfound{%
		\xs_ifnum{#1<1 }
			{\def\xs_reserved_A{#4}}
			{\xs_ifnum{\decimalpart>#1 }
				{\def\xs_reserved_A{#3}}
				{\def\xs_reserved_A{#4}}%
			}%
		\xs_eaddtomacro\xs_reserved_C{\xs_reserved_A}%
	}%
	\xs_ifempty{#3}%
		{\xs_exparg\xs_assign_xstringresult{\xs_reserved_D}{#5}%
		}
		{\xs_read_reserved_D
		\xs_exparg\xs_assign_xstringresult{\xs_reserved_C}{#5}%
		}%
}

% Supprime les #1 premières occurrences de #3 dans #2
\xs_newmacro\StrDel{0}{2}{1}{\xs_StrSubstitute[#1]{#2}{#3}{}[#4]}

\def\xs_exitallgroups{\ifnum\xs_nestlevel>0 \endgroup\expandafter\xs_exitallgroups\fi}

% Compte combien d'unités syntaxiques contient la chaine #1 ?
\xs_newmacro\StrLen{}{1}{1}{%
	\def\xs_reserved_C{#1}\decimalpart0 \def\xs_nestlevel{0}\gdef\groupID{0}%
	\let\xs_atbegingroup\relax
	\def\xs_atendofgroup{\expandafter\endgroup\expandafter\decimalpart\number\decimalpart\relax}%
	\let\xs_atnextsyntaxunit\relax
	\xs_read_reserved_C
	\xs_exparg\xs_assign_xstringresult{\number\decimalpart}{#2}%
}

% Macro interne fermant autant de groupes que nécessaire pour trouver une unité syntaxique derrière
\def\xs_continuetonext{%
	\xs_exparg\xs_ifempty{\xs_reserved_C}%
		{\ifnum\xs_nestlevel>0
			\xs_endgroup_eaddtomacro\xs_reserved_B{\expandafter{\xs_reserved_B}}% on concatène
			\expandafter\xs_continuetonext% on recommence
		\fi}
		{}%
}%

\def\xs_calc_grouIP{%
	\begingroup\def\xs_reserved_A{0}%
	\xs_ifx{\xs_reserved_A\groupID}% si on arrive du groupe de niveau 0
		{\endgroup\xdef\groupID{\number\integerpart}}% on met simplement le niveau
		{\endgroup\xs_eearg{\gdef\groupID}{\expandafter\groupID\expandafter,\number\integerpart}}%
}

% Cette macro coupe la chaine #1 après l'unité syntaxique n°#2
\def\StrSplit{%
	\xs_ifstar
		{\let\xs_reserved_E\xs_continuetonext\StrSplit_i}%
		{\let\xs_reserved_E\relax\StrSplit_i}%
}

\xs_newmacro\StrSplit_i{}{2}{0}{\xs_StrSplit_ii{#2}{#1}\xs_StrSplit_iii}

% Cette macro interne coupe la chaine #2 après l'unité syntaxique n°#1
% Le début est assigné dans \xs_reserved_B et la fin dans \xs_reserved_C
\long\def\xs_StrSplit_ii#1#2{%
	\let\xs_reserved_B\empty\def\xs_reserved_C{#2}\def\xs_reserved_D{#1}\gdef\groupID{}%
	\ifnum#1>0
		\decimalpart0 \integerpart0 \gdef\groupID{0}\def\xs_nestlevel{0}%
		\def\xs_atendofgroup{%
			\edef\__temp{%
				\endgroup
				\noexpand\decimalpart=\number\decimalpart\relax
				\unexpanded{\xs_addtomacro\xs_reserved_B}{{\unexpanded\expandafter{\xs_reserved_B}}}%
				}%
			\__temp
		}%
		\def\xs_atbegingroup{\let\xs_reserved_B\empty}%
		\def\xs_atnextsyntaxunit{%
			\xs_eaddtomacro\xs_reserved_B{\xs_reserved_A}%
			\xs_ifnum{\decimalpart=\xs_reserved_D\relax}
				{\ifx\xs_reserved_C\empty\xs_reserved_E\fi
				\edef\__temp{\def\noexpand\xs_reserved_B{\unexpanded\expandafter{\xs_reserved_B}}\def\noexpand\xs_reserved_C{\unexpanded\expandafter{\xs_reserved_C}}}%
				\expandafter\xs_exitallgroups\__temp
				\xs_gobarg% mange l'appel récursif \xs_read_reserved_C dans \xs_read_reserved_C
				}
				{}%
		}%
		\xs_read_reserved_C
	\fi
}

\def\xs_StrSplit_iii#1#2{\let#1\xs_reserved_B\let#2\xs_reserved_C}

% StrCut[n]{<texte>}{<motif>}\macroA\macroB
% \macroA reçoit ce qui se trouve avant la n ème occurrence <motif> dans <texte>
% \macroB reçoit ce qui est après cette n ème occurrence
\xs_newmacro*3\StrCut{1}{2}{0}{%
	\xs_ifempty{#3}%
		{\gdef\groupID{}\let\xs_reserved_C\empty\let\xs_reserved_E\empty
		}
		{\xs_ifnum{#1<1 }
			{\xs_StrCut_ii{#2}{#3}1}
			{\xs_StrCut_ii{#2}{#3}{#1}}%
		}%
	\xs_StrCut_iii
}

\long\def\xs_StrCut_ii#1#2#3{%
	\let\xs_reserved_C\empty\def\xs_reserved_D{#1}\def\xs_reserved_E{#2}%
	\decimalpart0 \integerpart0 \gdef\groupID{0}\def\xs_nestlevel{0}%
	\def\xs_atoccurfound{%
		\xs_ifnum{\decimalpart=\numexpr(#3)\relax}
			{\edef\__temp{%
				\def\noexpand\xs_reserved_C{\unexpanded\expandafter{\xs_reserved_C}}%
				\def\noexpand\xs_reserved_D{\unexpanded\expandafter{\xs_reserved_D}}%
				\noexpand\decimalpart=\number\decimalpart\relax
				}%
			\expandafter\xs_exitallgroups\__temp
			\xs_gobarg% stoppe la récursivité dans \xs_read_reserved_D
			}
			{\xs_eaddtomacro\xs_reserved_C{\xs_reserved_E}%
			}%
	}%
	\xs_read_reserved_D
	\let\xs_reserved_E\xs_reserved_D
	\xs_exparg{\def\xs_reserved_D}{\xs_reserved_C#2}%
}

\long\def\xs_StrCut_iii#1#2{\let#1\xs_reserved_C\let#2\xs_reserved_E}

% De la chaine #1, renvoie ce qui se trouve entre les positions
%  #2 et #3, unités syntaxiques aux positions compris !
\xs_newmacro\StrMid{}{3}{1}{%
	\begingroup
		\noexploregroups
		\let\xs_reserved_E\relax
		\xs_StrSplit_ii{#3}{#1}%
		\edef\xs_reserved_C{\number\numexpr#2-1}%
		\let\xs_reserved_E\relax
		\xs_exptwoargs\xs_StrSplit_ii\xs_reserved_C\xs_reserved_B
	\expandafter\endgroup
	\expandafter\xs_assign_xstringresult\expandafter{\xs_reserved_C}{#4}%
	\gdef\groupID{}%
}

% supprime #2 unités syntaxiques à gauche dans la chaine #1
\xs_newmacro\StrGobbleLeft{}{2}{1}{%
	\let\xs_reserved_E\relax
	\xs_StrSplit_ii{#2}{#1}%
	\xs_exparg\xs_assign_xstringresult{\xs_reserved_C}{#3}%
}

% extrait de #1 la chaine à gauche de longueur #2
\xs_newmacro\StrLeft{}{2}{1}{%
	\let\xs_reserved_E\relax
	\xs_StrSplit_ii{#2}{#1}%
	\xs_exparg\xs_assign_xstringresult{\xs_reserved_B}{#3}%
}

% supprime #2 unités syntaxiques à droite dans la chaine #1
\xs_newmacro\StrGobbleRight{}{2}{1}{%
	\xs_StrLen{#1}[\xs_reserved_D]%
	\let\xs_reserved_E\relax
	\xs_exparg\xs_StrSplit_ii{\number\numexpr\xs_reserved_D-#2}{#1}%
	\xs_exparg\xs_assign_xstringresult{\xs_reserved_B}{#3}%
}

% renvoie #2 unités syntaxiques à la droite de la chaine #1
\xs_newmacro\StrRight{}{2}{1}{%
	\xs_StrLen{#1}[\xs_reserved_D]%
	\let\xs_reserved_E\relax
	\xs_exparg\xs_StrSplit_ii{\number\numexpr\xs_reserved_D-#2}{#1}%
	\xs_exparg\xs_assign_xstringresult{\xs_reserved_C}{#3}%
}

\xs_newmacro\StrChar{}{2}{1}{%
	\let\xs_reserved_B\empty\def\xs_reserved_C{#1}\def\xs_reserved_D{#2}%
	\ifnum#2>0
		\def\groupID{0}\def\xs_nestlevel{0}\integerpart0 \decimalpart0
		\let\xs_atbegingroup\relax
		\def\xs_atendofgroup{\expandafter\endgroup\expandafter\decimalpart\number\decimalpart\relax}%
		\def\xs_atnextsyntaxunit{%
			\ifnum\decimalpart=\xs_reserved_D% la n ième US est atteinte ?
				\edef\__temp{\def\noexpand\xs_reserved_B{\unexpanded\expandafter{\xs_reserved_A}}}% on capture l'US en cours qui est celle cherchée
				\expandafter\xs_exitallgroups\__temp
				\expandafter\xs_gobarg% stoppe la récursivité dans \xs_read_reserved_C
			\fi
		}%
		\xs_read_reserved_C
	\fi
	\xs_exparg\xs_ifempty{\xs_reserved_B}%
		{\gdef\groupID{}}
		{}%
	\xs_exparg\xs_assign_xstringresult{\xs_reserved_B}{#3}%
}

% Combien de fois compte t-on #2 dans #1 ?
\xs_newmacro\StrCount{}{2}{1}{%
	\def\xs_reserved_D{#1}\def\xs_reserved_E{#2}\let\xs_reserved_C\empty
	\xs_ifempty{#2}%
		{\xs_assign_xstringresult{0}{#3}%
		}
		{\decimalpart0 \integerpart0 \gdef\groupID{0}\def\xs_nestlevel{0}%
		\def\xs_atoccurfound{\let\xs_reserved_C\empty\xs_read_reserved_D}%
		\xs_read_reserved_D
		\xs_exparg\xs_assign_xstringresult{\number\decimalpart}{#3}%
		}%
}

% renvoie la position de l'occurrence #1 de la sous chaine #3 dans la chaine #2
\xs_newmacro\StrPosition{1}{2}{1}{%
	\xs_cutafteroccur{#2}{#3}{#1}%
	\let\xs_reserved_E\groupID
	\xs_ifx{\xs_reserved_C\xs_reserved_D}
		{\xs_assign_xstringresult{0}{#4}%
		\let\xs_reserved_E\empty
		}
		{\xs_exparg\xs_StrLen{\xs_reserved_C}[\xs_reserved_C]%
		\xs_exparg\xs_assign_xstringresult{\number\numexpr\xs_reserved_C+1}{#4}%
		}%
	\global\let\groupID\xs_reserved_E
}

\def\comparestrict{\def\xs_comparecoeff{1}}
\def\comparenormal{\def\xs_comparecoeff{0}}
\def\savecomparemode{\let\xs_saved_comparecoeff\xs_comparecoeff}
\def\restorecomparemode{\let\xs_comparecoeff\xs_saved_comparecoeff}

% Compare les deux arguments #1 et #2
% Renvoie 0 s'ils sont égaux et renvoie la
% position de la premiere unité syntaxiques différente sinon
\xs_newmacro*2\StrCompare{}{2}{1}{%
	\def\xs_reserved_A{#1}%
	\def\xs_reserved_B{#2}%
	\xs_ifx{\xs_reserved_B\xs_reserved_A}
		{\xs_assign_xstringresult{0}{#3}}
		{\xs_StrCompare_i{#1}{#2}{#3}}%
}

\long\def\xs_StrCompare_i#1#2#3{%
	\def\xs_StrCompare_iii##1{%
		\let\xs_reserved_A\empty
		\xs_exparg\xs_ifempty{\xs_reserved_C}%
			{\edef\xs_reserved_A{*\xs_comparecoeff}}%
			{\xs_exparg\xs_ifempty{\xs_reserved_D}%
				{\edef\xs_reserved_A{*\xs_comparecoeff}}
				{}%
			}%
		\def\xs_next{\xs_exparg\xs_assign_xstringresult{\number\numexpr##1\xs_reserved_A\relax}{#3}}%
	}%
	\def\xs_StrCompare_ii##1{% ##1 est la position
		\xs_exparg\xs_returnfirstsyntaxunit{\xs_reserved_C}\xs_reserved_A
		\xs_exparg\xs_returnfirstsyntaxunit{\xs_reserved_D}\xs_reserved_B
		\xs_ifx{\xs_reserved_B\xs_reserved_A}
			{\xs_exparg\xs_ifempty{\xs_reserved_A}%
				{\xs_StrCompare_iii{##1}% les 2 unités syntaxiques sont égales, on renvoie la position
				}
				{\def\xs_next{\xs_exparg\xs_StrCompare_ii{\number\numexpr##1+1}}% les 2 unités syntaxiques sont égales et non vides, on recommence
				\xs_exparg\xs_removefirstsyntaxunit{\xs_reserved_C}\xs_reserved_C
				\xs_exparg\xs_removefirstsyntaxunit{\xs_reserved_D}\xs_reserved_D
				}%
			}% les 2 unités syntaxiques sont différentes : on renvoie la position
			{\xs_StrCompare_iii{##1}%
			}%
		\xs_next
	}%
	\def\xs_reserved_C{#1}\def\xs_reserved_D{#2}%
	\xs_StrCompare_ii1%
}

\xs_newmacro\StrFindGroup{}{2}{1}{%
	\def\xs_reserved_A{#2}\def\xs_reserved_B{0}%
	\xs_ifx{\xs_reserved_A\xs_reserved_B}
		{\xs_assign_xstringresult{{#1}}{#3}}
		{\xs_StrFindGroup_i{#1}{#2}[#3]}%
}

\long\def\xs_StrFindGroup_i#1#2[#3]{%
	\def\xs_StrFindGroup_ii{%
		\xs_exparg\xs_ifempty{\xs_reserved_C}%
			{\xs_assign_xstringresult{}{#3}% s'il ne reste plus rien, on renvoie vide
			}
			{\xs_exparg\xs_returnfirstsyntaxunit{\xs_reserved_C}\xs_reserved_D
			\xs_ifx{\bgroup\xs_toks}% si la 1ère unité syntaxique est un groupe explicite
				{\advance\decimalpart1 % on augmente le compteur
				\xs_ifnum{\decimalpart=\xs_reserved_A\relax}% on est au groupe cherché lors de la profondeur courante ?
					{\xs_ifx{\empty\xs_reserved_B}% on est à la profondeur maximale ?
						{\xs_exparg\xs_assign_xstringresult{\xs_reserved_D}{#3}}% on renvoie ce groupe
						{\xs_exparg{\expandafter\xs_StrFindGroup_i\xs_reserved_D}{\xs_reserved_B}[#3]}% on recommence avec ce groupe et les profondeurs de recherche restantes
					}
					{\xs_exparg\xs_removefirstsyntaxunit{\xs_reserved_C}\xs_reserved_C
					\xs_StrFindGroup_ii
					}%
				}
				{\xs_exparg\xs_removefirstsyntaxunit{\xs_reserved_C}\xs_reserved_C
				\xs_StrFindGroup_ii
				}%
			}%
	}%
	\xs_extractgroupnumber{#2}\xs_reserved_A\xs_reserved_B
	\decimalpart0
	\xs_ifnum{\xs_reserved_A>0 }
		{\def\xs_reserved_C{#1}}
		{\let\xs_reserved_C\empty}%
	\xs_StrFindGroup_ii
}

\def\xs_extractgroupnumber#1#2#3{%
	\def\xs_extractgroupnumber_i##1,##2\_nil{\def#2{##1}\def#3{##2}}%
	\xs_extractgroupnumber_i#1,\_nil
	\ifx\empty#3\else\xs_extractgroupnumber_i#1\_nil\fi
}

\def\expandingroups{\let\xs_expandingroups\exploregroups}

\def\noexpandingroups{\let\xs_expandingroups\noexploregroups}

\def\StrExpand{\xs_testopt{\xs_StrExpand}{1}}
\long\def\xs_StrExpand[#1]#2#3{%
	\begingroup
		\xs_expandingroups
		\xs_ifnum{#1>0 }
			{\integerpart#1 \decimalpart0 \gdef\groupID{0}\def\xs_nestlevel{0}%
			\def\xs_atendofgroup{\xs_endgroup_eaddtomacro\xs_reserved_B{\expandafter{\xs_reserved_B}}}%
			\def\xs_atbegingroup{\let\xs_reserved_B\empty}%
			\def\xs_atnextsyntaxunit{\xs_eeaddtomacro\xs_reserved_B{\xs_reserved_A}}%
			\def\xs_reserved_C{#2}%
			\xs_StrExpand_i{#1}% Appel de la macro récursive
			}
			{\def\xs_reserved_B{#2}%
			}
		\expandafter
	\endgroup
	\expandafter\def\expandafter#3\expandafter{\xs_reserved_B}%
	\gdef\groupID{}%
}

\long\def\xs_StrExpand_i#1{%
	\xs_ifnum{#1>0 }
		{\let\xs_reserved_B\empty
		\xs_read_reserved_C
		\let\xs_reserved_C\xs_reserved_B
		\def\xs_reserved_A{\xs_exparg\xs_StrExpand_i{\number\numexpr#1-1}}%
		}
		{\let\xs_reserved_A\relax
		}%
	\xs_reserved_A
}

\def\scancs{\xs_testopt{\xs_scancs}{1}}
\long\def\xs_scancs[#1]#2#3{%
	\xs_StrExpand[#1]{#3}{#2}%
	\edef#2{\detokenize\expandafter{#2}}%
}

\restorexstringcatcode

\setverbdelim{|}%
\fullexpandarg\saveexpandmode
\comparenormal\savecomparemode
\noexploregroups\saveexploremode
\expandingroups

\endinput

                        H I S T O R I Q U E
------------------------------------------------------------------------------
v1.0    4/7/2008 : - Package achevé.
         7/7/2008 : - Package publié sur CTAN.
------------------------------------------------------------------------------
v1.1    15/8/2008
   - Le package ne nécessite plus LaTeX et est désormais utilisable sous
     Plain eTeX.
   - Ajout des macros \IfInteger et \IfDecimal.
     Pour cette dernière, la partie entière et la partie décimale sont
     récupérables dans les compteurs \integerpart et \decimalpart. Ce
     qu'il reste après qu'un caractère non attendu soit rencontré est
     dispo dans \xs_remainafterdecimal
   - Correction d'un bug dans \tokenize :
        suppression de l'expansion avec \normalexpandarg pour éviter le bug
        avec les lettres accentuées dans l'exemple : \tokenize\aa{éù}
   - Amélioration du code de la plupart des macros.
   - écriture d'une routine \xs_newmacro définissant les  macros.
   - Suppression de tous les compteurs grace à \numexpr.
   - Nouvelles fonctionnalités internes dans :
      \IfSubStr
        ajout des chaines se trouvant avant et après l'occurrence testée
        dans les sc \xs_behind_IfSubStr et \xs_before_IfSubStr
      \StrCount
        a) ajout de ce qui se trouve après la dernière occurrence dans la
           sc \xs_StrCount_afterlastocccur
        b) la macro ne dépend plus d'aucune autre
------------------------------------------------------------------------------
v1.2    23/8/2008
   - Amélioration du code de \StrMid \StrGobbleLeft, \StrLeft,
     \StrGobbleRight et \StrRight à l'aide de la nouvelle macro
     \xs_StrSplit_i
   - Nouveau test \IfStrEq qui compare 2 chaines
   - Nouveau test \IfEq qui compare 2 chaines (ou 2 nombres si les 2 chaines
     contiennent un nombre)
   - Correction d'un bug dans \xs_formatnumber. La macro n'envisageait pas le
     cas où son argument était vide ce qui faiasait planter
     \IfDecimal{}{V}{F} et \IfInteger{}{V}{F}
------------------------------------------------------------------------------
v1.3    21/9/2008
  - Amélioration du code, mise en place de récursivités terminales dans
    toutes les macros récursives, simplification de \xs_TestEqual en
    utilisant \ifx
  - Nouvelles macros \IfStrEqCase et \IfEqCase
      Teste si une chaîne est égale à plusieurs chaines données et
      exécute un code spécifique
  - Création de la macro publique \StrSplit
      Coupe la chaine en 2 à une position donnée
  - Nouvelle macro \StrCompare
      Compare 2 chaînes et renvoie la position du 1er caractère différent.
      Renvoie 0 si elles sont égales.
------------------------------------------------------------------------------
v1.3a   29/9/2008
  - Correction d'un bug : \expandafter#1
    dans les macros \IfSubStrBefore et \StrBetween qui buggue si #1 est un
    nombre > 9 !
  - Ré écriture de \xs_returnfirstsyntaxunit et \xs_gobarg qui
    deviennent purement développables.
  - Ré écriture de \StrLen
  - Nouvelle macro interne \xs_cutafteroccur
      Coupe la chaine après la nième occurrence d'une sous chaine.
  - Code amélioré de \StrMid, \StrLeft, \StrGobbleLeft, \StrRight,
    \StrGobbleRight grace à \xs_cutafteroccur
------------------------------------------------------------------------------
v1.4   4/11/2008
  - xstring traite ses arguments par unité syntaxique, et donc toutes les
    macros internes ont été ré-écrites à cette fin.
  - Le manuel a été ré-écrit, rendu plus clair et mieux structuré.
  - Nouvelle fonctionnalité : \expandarg
      le 1er lexème de chaque argument est 1-développé avant que la
      macro ne soit appelée. Si un argument comporte plus qu'1 lexème,
      il faut passer par \scancs*[1] pour 1-développer toutes les unités
      syntaxiques.
  - Correction de 2 erreurs dans le manuel anglais :  0 est la valeur par
    défaut dans \StrSubstitute et \StrDel
  - Cohérence dans les nom des séquences de contrôles temporaires qui
    sont désormais : \xs_reserved_A à \xs_reserved_E
------------------------------------------------------------------------------
v1.4a  12/11/2008
  - Correction d'un bug dans \xs_StrSplit dans le cas où l'argument
     numérique est <1 : la 1ere coupure doit être vide et le seconde doit
     être égale à l'argument.
------------------------------------------------------------------------------
v1.4b  16/11/2008
  - Correction de 2 bugs dans \xs_returnfirstsyntaxunit
------------------------------------------------------------------------------
v1.5   31/12/2008
  - Nouvelles fonctionnalités dans la recherche de groupes par un
    identificateur caractérisant leur imbrication. Implémentation de :
      1) \StrFindGroup
      2) \groupID
  - Ajout des nouvelles macros génériques \xs_read_reserved_C et
    \xs_read_reserved_D
  - Correction d'un bug dans \StrSplit : \StrSplit{{a}bc}{1}[\truc] faisait
    que \truc contenait «a{a}».
  - Correction d'un bug dans \xs_newmacro : l'argument optionnel était
    détokénisé à tort dans les macros étoilées.
  - Dans \xs_newmacro, on doit choisir le numéro du dernier argument devant
    être détokénisé dans le cas d'une macro étoilée (sachant que
     l'argument optionnel ne l'est jamais)
------------------------------------------------------------------------------
v1.5a  09/2/2009
  - Nouvelle macro \StrExpand, sensible au mode d'exploration. La macro est
    indépendante du mode d'exploration et dispose de ses propres commandes
    d'exploration : \expandingroups et \noexpandingroups
  - Ré-écriture de \scancs, qui devient triviale puisque dépendant de
    \StrExpand. Il n'y a plus de version étoilée et désormais, \scancs
    est sensible au mode d'exploration.
  - Correction d'un bug dans \IfInteger : \IfInteger{2.0}{V}{F} affichait F
  - Correction de bugs : mettre \let\xs_reserved_E\relax avant d'appeler
    \xs_StrSplit_i
  - Suppression des messages d'erreur, de warning et d'info. xstring devient
    donc silencieux ;)
  - Passage de 3 à 2 compteurs
  - Le manuel est désormais plus coloré, en espérant qu'il sera un peu
    plus agréable à lire !
------------------------------------------------------------------------------
v1.5b  13/3/2009
  - Modification d'un grand nombre de macros de telle sorte que vraiment
    n'importe quel code peut désormais être placé dans les arguments des
    macros (comme par exemple des \if, \ifx ou autre, même sans leur \fi, ce
    qui n'était pas possible jusqu'alors)
------------------------------------------------------------------------------
v1.5c  05/6/2009
  - Correction d'un bug dans \IfBeginWith : il faut appeler
    \xs_returnfirstsyntaxunit pour l'argument #2 puis pour l'argument #1 et
    non pas l'inverse pour que \xs_toks reflète ce qui se trouve dans #1
  - Correction d'un bug dans \xs_returnfirstsyntaxunit au cas où #1 commence
    par un espace : mettre \xs_toks à 0
  - Correction d'un bug dans \xs_returnfirstsyntaxunit :
    \xs_returnfirstsyntaxunit{{}}\truc
    faisait que \truc se développait en un espace.
  - Correction d'un bug dans \xs_removefirstsyntaxunit où le cas
    \xs_removefirstsyntaxunit{ {b}}\truc
    donnait \truc se développant en «b» au lieu de «{b}».
------------------------------------------------------------------------------
v1.5d  28/3/2010
  - Correction d'un bug dans \IfInteger : \afterinteger ne donnait pas le
    bon résultat. Par exemple avec 1.23 il renvoyait {} au lieu de {.23}
  - \xs_formatnumber ne detokenize plus ses arguments (que m'est-il passé
    par la tête pour que je code un truc comme ca ?), et donc
    \afterinteger et \xs_afterdecimal ont des tokens ayant le bon
    catcode
------------------------------------------------------------------------------
v1.6  24/10/2012
  - Correction d'un bug dans \xs_cutafteroccur au cas où #3<1
  - \IfDecimal ne \detokenize plus l'argument.
  - Nouvelle version de \tokenize qui enlevait les accolades si son argument
    était entre accolades
  - Nouvelle macro \StrCut
  - \xs_cutafteroccur_i ne produit plus d'espace indésirable si #3 était
    évalué par \numexpr
------------------------------------------------------------------------------
v1.7  13/1/2013
  - Correction d'un manque de rigueur dans les assignations concernant
    \groupID : elles sont toutes globales désormais
  - Les macros de xstring sont \long
------------------------------------------------------------------------------
v1.7a 28/2/2013
  - Correction d'un espace parasite dans \xs_removefirstsyntaxunit
------------------------------------------------------------------------------
v1.7b 29/7/2013
  - La date contenue dans \xstringdate est désormais conforme
------------------------------------------------------------------------------
v1.7c 13/10/2013
  - les macros impliquées dans \IfStrCase et \IfStrEqCase sont désormais \long
------------------------------------------------------------------------------
v1.8  07/12/2018
  - affectations globales supprimées (sauf pour \groupID) afin de ne pas
    surcharger la pile de sauvegarde
  - nettoyage du code, corrections de lourdeurs et maladresses
------------------------------------------------------------------------------
v1.81 09/12/2018
  - bug dans \IfInteger et \IfDecimal, la macro \xs_afterdecimal est indéfinie
    et doit être remplacée par \afterdecimal
------------------------------------------------------------------------------
v1.82 01/02/2019
  - \xs_testopt n'est pas longue et provoque un bug dans \xs_IfStrCase et
    \xs_IfStrCase lorsque #1 contient \par : \xs_testopt reste courte et
    \xs_IfStringCase a été modifiée pour que cela fonctionne.
    ------------------------------------------------------------------------------
v1.83 06/02/2019
      - mauvaise approche et mauvais fix dans la v1.82 : \xs_testopt devient
        longue, pas le choix (et donc aussi \xs_ifnxttok)

==> xstring/test_etex.tex <==
%##################### WARNING #####################
% This is NOT a LaTeX file, it is a TeX file.
% It must be compiled with eTeX typing <etex test_etex>
%#################### ATTENTION ####################
% Ceci n'est PAS un fichier LaTeX, c'est un fichier TeX.
% Il doit être compilé avec eteX en tapant <etex test_etex>
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input xstring
\def\delimiteur{-{}}
\font\hugerm=ecbx2000
\font\hugett=ectt1750
\font\largeboldrm=ecbx1300
\font\largett=ectt1300
\font\textfont=ecrm1000
\textfont
\catcode`\@=11\relax
\gdef\exemple{\csname xs_ifstar\endcsname{\def\frontiere{\delimiteur}\csname xs_toks_toverb\endcsname}{\def\frontiere{}\csname xs_toks_toverb\endcsname}}
\expandafter\def\csname xs_assign_verb\endcsname#1{%
	\noexpandarg
	\tokenize\cs@resultat{#1}%
	\fullexpandarg
	\leavevmode\hbox to0.7\hsize{\hfil\tt#1}\quad\frontiere\cs@resultat\frontiere\hfil\par}%
\catcode`\@=12\relax
\def\chapitre#1#2{\vskip 6pt plus 2pt minus 2pt{{\largeboldrm#1} {\largett#2}}\vskip 3pt plus 1pt minus 1pt}
\def\AvecArgOptionnel{\vskip 6pt plus 2pt minus 2pt Mêmes exemples avec l'argument optionnel :\par}
\hoffset-1.54cm\hsize19cm\parindent0pt
% debut du texte
\hfil{\hugerm Ceci est le fichier de test de xstring}\hfil{}

\hrule\vskip0.5ex

\hrule\vskip2ex

Attention : ce fichier {\tt test\_etex.tex} produit une sortie quasiment identique au fichier {\tt test\_latex.tex}, mais il doit se lancer avec Plain $\varepsilon$-\TeX. Pour des raison d'encodage, contrairement au fichier {\tt test\_latex.tex}, les arguments des macros présentées ici ne contiennent pas de lettres accentuées.\vskip2em

Toutes les situations ne sont pas envisagées, mais au moins un grand nombre ! Les macros sont examinées dans l'ordre logique du code.

Lorsque le résultat contient des espaces ou peut conduire à des doutes, il sera entouré de ''\delimiteur``, étant entendu que ''\delimiteur\delimiteur`` est une chaine vide.\vskip2em

\hfill{\hugerm Le mode \hugett\string\fullexpandarg}\hfill{}

\vskip-1ex\hfil\hbox to8cm{\hrulefill}\hfil{}\vskip3.5ex

\chapitre{Le test}{IfSubStr}

\exemple|\IfSubStr{abcdef}{cd}{vrai}{faux}|
\exemple|\IfSubStr{a b c d }{b c}{vrai}{faux}|
\exemple|\IfSubStr{a b c d }{bc}{vrai}{faux}|
\exemple|\IfSubStr{abcdef}{}{vrai}{faux}|
\exemple|\IfSubStr{a}{a}{vrai}{faux}|
\exemple|\IfSubStr{aaaa}{aa}{vrai}{faux}|
\exemple|\IfSubStr{a}{aa}{vrai}{faux}|
\exemple|\IfSubStr{a}{}{vrai}{faux}|
\exemple|\IfSubStr{}{a}{vrai}{faux}|
\exemple|\IfSubStr{}{}{vrai}{faux}|
\exemple|\IfSubStr[2]{abaca}{a}{vrai}{faux}|
\exemple|\IfSubStr[3]{abaca}{a}{vrai}{faux}|
\exemple|\IfSubStr[4]{abaca}{a}{vrai}{faux}|
\exemple|\IfSubStr[-2]{abaca}{a}{vrai}{faux}|

\chapitre{Le test}{IfBeginWith}

\exemple|\IfBeginWith{abcdef}{adc}{vrai}{faux}|
\exemple|\IfBeginWith{abcdef}{abcd}{vrai}{faux}|
\exemple|\IfBeginWith{ a b c }{ a}{vrai}{faux}|
\exemple|\IfBeginWith{a b c d}{ab}{vrai}{faux}|
\exemple|\IfBeginWith{a}{a}{vrai}{faux}|
\exemple|\IfBeginWith{a}{aa}{vrai}{faux}|
\exemple|\IfBeginWith{a}{}{vrai}{faux}|
\exemple|\IfBeginWith{}{a}{vrai}{faux}|
\exemple|\IfBeginWith{}{}{vrai}{faux}|

\chapitre{Le test}{IfEndWith}

\exemple|\IfEndWith{abcdef}{ab}{vrai}{faux}|
\exemple|\IfEndWith{abcdef}{f}{vrai}{faux}|
\exemple|\IfEndWith{ a b c }{c}{vrai}{faux}|
\exemple|\IfEndWith{ a b c }{ }{vrai}{faux}|
\exemple|\IfEndWith{a}{a}{vrai}{faux}|
\exemple|\IfEndWith{a}{aa}{vrai}{faux}|
\exemple|\IfEndWith{a}{}{vrai}{faux}|
\exemple|\IfEndWith{}{a}{vrai}{faux}|
\exemple|\IfEndWith{}{}{vrai}{faux}|

\chapitre{Le test}{IfSubStrBefore}

\exemple|\IfSubStrBefore{abcdef}{b}{e}{vrai}{faux}|
\exemple|\IfSubStrBefore{abcdef}{e}{c}{vrai}{faux}|
\exemple|\IfSubStrBefore{ a b c }{ }{b}{vrai}{faux}|
\exemple|\IfSubStrBefore{ a b c }{ b}{c }{vrai}{faux}|
\exemple|\IfSubStrBefore{abcdef}{z}{a}{vrai}{faux}|
\exemple|\IfSubStrBefore{abcdef}{y}{z}{vrai}{faux}|
\exemple|\IfSubStrBefore{abcdef}{a}{z}{vrai}{faux}|
\exemple|\IfSubStrBefore{aaa}{a}{aa}{vrai}{faux}|
\exemple|\IfSubStrBefore{abcdef}{a}{a}{vrai}{faux}|
\exemple|\IfSubStrBefore{a}{a}{a}{vrai}{faux}|
\exemple|\IfSubStrBefore{}{a}{b}{vrai}{faux}|
\exemple|\IfSubStrBefore{a}{}{a}{vrai}{faux}|
\exemple|\IfSubStrBefore{}{a}{a}{vrai}{faux}|
\exemple|\IfSubStrBefore{}{}{}{vrai}{faux}|
\exemple|\IfSubStrBefore[1,1]{abacada}{d}{a}{vrai}{faux}|
\exemple|\IfSubStrBefore[1,2]{abacada}{d}{a}{vrai}{faux}|
\exemple|\IfSubStrBefore[1,3]{abacada}{d}{a}{vrai}{faux}|
\exemple|\IfSubStrBefore[1,4]{abacada}{d}{a}{vrai}{faux}|
\exemple|\IfSubStrBefore[2,1]{maman papa}{a}{p}{vrai}{faux}|
\exemple|\IfSubStrBefore[2,2]{maman papa}{a}{p}{vrai}{faux}|
\exemple|\IfSubStrBefore[4,2]{maman papa}{a}{p}{vrai}{faux}|

\chapitre{Le test}{IfStrBehind}

\exemple|\IfSubStrBehind{abcdef}{b}{e}{vrai}{faux}|
\exemple|\IfSubStrBehind{abcdef}{e}{c}{vrai}{faux}|
\exemple|\IfSubStrBehind{ a b c }{ }{b}{vrai}{faux}|
\exemple|\IfSubStrBehind{ a b c }{ c}{ a}{vrai}{faux}|
\exemple|\IfSubStrBehind{abcdef}{z}{a}{vrai}{faux}|
\exemple|\IfSubStrBehind{abcdef}{y}{z}{vrai}{faux}|
\exemple|\IfSubStrBehind{abcdef}{a}{z}{vrai}{faux}|
\exemple|\IfSubStrBehind{aaa}{a}{aa}{vrai}{faux}|
\exemple|\IfSubStrBehind{abcdef}{a}{a}{vrai}{faux}|
\exemple|\IfSubStrBehind{a}{a}{a}{vrai}{faux}|
\exemple|\IfSubStrBehind{}{a}{b}{vrai}{faux}|
\exemple|\IfSubStrBehind{a}{}{a}{vrai}{faux}|
\exemple|\IfSubStrBehind{}{a}{a}{vrai}{faux}|
\exemple|\IfSubStrBehind{}{}{}{vrai}{faux}|
\exemple|\IfSubStrBehind[1,1]{abacada}{c}{a}{vrai}{faux}|
\exemple|\IfSubStrBehind[1,2]{abacada}{c}{a}{vrai}{faux}|
\exemple|\IfSubStrBehind[1,3]{abacada}{c}{a}{vrai}{faux}|
\exemple|\IfSubStrBehind[2,1]{maman papa}{a}{p}{vrai}{faux}|
\exemple|\IfSubStrBehind[3,1]{maman papa}{a}{p}{vrai}{faux}|
\exemple|\IfSubStrBehind[3,2]{maman papa}{a}{p}{vrai}{faux}|
\exemple|\IfSubStrBehind[4,2]{maman papa}{a}{p}{vrai}{faux}|

\chapitre{Le test}{IfInteger}

\exemple|\IfInteger{156}{vrai}{faux}|
\exemple|\IfInteger{1.6}{vrai}{faux}|
\exemple|\IfInteger{7a5}{vrai}{faux}|
\exemple|\IfInteger{+9}{vrai}{faux}|
\exemple|\IfInteger{-15}{vrai}{faux}|
\exemple|\IfInteger{0}{vrai}{faux}|
\exemple|\IfInteger{-1,2}{vrai}{faux}|
\exemple|\IfInteger{1.}{vrai}{faux}|
\exemple|\IfInteger{-00}{vrai}{faux}|
\exemple|\IfInteger{+}{vrai}{faux}|
\exemple|\IfInteger{-}{vrai}{faux}|
\exemple|\IfInteger{.}{vrai}{faux}|
\exemple|\IfInteger{}{vrai}{faux}|

\chapitre{Le test}{IfDecimal}

\exemple|\IfDecimal{6}{vrai}{faux}|
\exemple|\IfDecimal{-78}{vrai}{faux}|
\exemple|\IfDecimal{3.14}{vrai}{faux}|
\exemple|\IfDecimal{3,14}{vrai}{faux}|
\exemple|\IfDecimal{1..5}{vrai}{faux}|
\exemple|\IfDecimal{-9.8}{vrai}{faux}|
\exemple|\IfDecimal{+9.8}{vrai}{faux}|
\exemple|\IfDecimal{-9,8}{vrai}{faux}|
\exemple|\IfDecimal{+9,8}{vrai}{faux}|
\exemple|\IfDecimal{+6.7.}{vrai}{faux}|
\exemple|\IfDecimal{.5}{vrai}{faux}|
\exemple|\IfDecimal{1.}{vrai}{faux}|
\exemple|\IfDecimal{-.99}{vrai}{faux}|
\exemple|\IfDecimal{-5.}{vrai}{faux}|
\exemple|\IfDecimal{5a9.}{vrai}{faux}|
\exemple|\IfDecimal{+}{vrai}{faux}|
\exemple|\IfDecimal{-}{vrai}{faux}|
\exemple|\IfDecimal{.}{vrai}{faux}|
\exemple|\IfDecimal{}{vrai}{faux}|

\chapitre{Le test}{IfStrEq}

\exemple|\IfStrEq{abcdef}{abcdef}{vrai}{faux}|
\exemple|\IfStrEq{a b c}{a b c}{vrai}{faux}|
\exemple|\IfStrEq{abcd}{abc}{vrai}{faux}|
\exemple|\IfStrEq{aab}{ab}{vrai}{faux}|
\exemple|\IfStrEq{aab}{aa}{vrai}{faux}|
\exemple|\IfStrEq{1.2}{1.20}{vrai}{faux}|
\exemple|\IfStrEq{3,4}{3.4}{vrai}{faux}|
\exemple|\IfStrEq{ }{  }{vrai}{faux}|
\exemple|\IfStrEq{}{a}{vrai}{faux}|
\exemple|\IfStrEq{a}{}{vrai}{faux}|
\exemple|\IfStrEq{}{}{vrai}{faux}|

\chapitre{Le test}{IfEq}

\exemple|\IfEq{abcdef}{abcdef}{vrai}{faux}|
\exemple|\IfEq{a b c}{a b c}{vrai}{faux}|
\exemple|\IfEq{abcd}{abc}{vrai}{faux}|
\exemple|\IfEq{aab}{ab}{vrai}{faux}|
\exemple|\IfEq{aab}{aa}{vrai}{faux}|
\exemple|\IfEq{1.2}{1.20}{vrai}{faux}|
\exemple|\IfEq{+1.0000}{1}{vrai}{faux}|
\exemple|\IfEq{-10}{10}{vrai}{faux}|
\exemple|\IfEq{1,2}{1.2}{vrai}{faux}|
\exemple|\IfEq{.5}{0.5}{vrai}{faux}|
\exemple|\IfEq{,5}{0,5}{vrai}{faux}|
\exemple|\IfEq{10}{dix}{vrai}{faux}|
\exemple|\IfEq{123}{1a3}{vrai}{faux}|
\exemple|\IfEq{0}{}{vrai}{faux}|
\exemple|\IfEq{++10}{+10}{vrai}{faux}|
\exemple|\IfEq{--10}{+10}{vrai}{faux}|
\exemple|\IfEq{a}{}{vrai}{faux}|
\exemple|\IfEq{}{a}{vrai}{faux}|
\exemple|\IfEq{}{}{vrai}{faux}|

\chapitre{La macro}{StrBefore}

\exemple|\StrBefore{abcedef}{e}|
\exemple*|\StrBefore{abcdef}{a}|
\exemple*|\StrBefore{abcdef}{z}|
\exemple*|\StrBefore{a b c d}{c}|
\exemple*|\StrBefore{a b c d}{ }|
\exemple*|\StrBefore[2]{a b c d}{ }|
\exemple*|\StrBefore[3]{a b c d}{ }|
\exemple*|\StrBefore[9]{a b c d}{ }|
\exemple*|\StrBefore[-7]{a b c d}{ }|
\exemple*|\StrBefore{abcdef}{Z}|
\exemple*|\StrBefore[1]{aaaaaa}{aa}|
\exemple|\StrBefore[2]{aaaaaa}{aa}|
\exemple|\StrBefore[3]{aaaaaa}{aa}|
\exemple*|\StrBefore[4]{aaaaaa}{aa}|
\exemple*|\StrBefore{a}{}|
\exemple*|\StrBefore{}{a}|
\exemple*|\StrBefore{}{}|

\AvecArgOptionnel
\exemple|\StrBefore{abcedef}{e}[\aa]\aa|
\exemple*|\StrBefore{abcdef}{a}[\aa]\aa|
\exemple*|\StrBefore{abcdef}{z}[\aa]\aa|
\exemple*|\StrBefore{a b c d}{c}[\aa]\aa|
\exemple*|\StrBefore{a b c d}{ }[\aa]\aa|
\exemple*|\StrBefore[2]{a b c d}{ }[\aa]\aa|
\exemple*|\StrBefore[3]{a b c d}{ }[\aa]\aa|
\exemple*|\StrBefore[9]{a b c d}{ }[\aa]\aa|
\exemple*|\StrBefore[-7]{a b c d}{ }[\aa]\aa|
\exemple*|\StrBefore{abcdef}{Z}[\aa]\aa|
\exemple*|\StrBefore[1]{aaaaaa}{aa}[\aa]\aa|
\exemple|\StrBefore[2]{aaaaaa}{aa}[\aa]\aa|
\exemple|\StrBefore[3]{aaaaaa}{aa}[\aa]\aa|
\exemple*|\StrBefore[4]{aaaaaa}{aa}[\aa]\aa|
\exemple*|\StrBefore{a}{}[\aa]\aa|
\exemple*|\StrBefore{}{a}[\aa]\aa|
\exemple*|\StrBefore{}{}[\aa]\aa|

\chapitre{La macro}{StrBehind}

\exemple|\StrBehind{abcedef}{e}|
\exemple*|\StrBehind{abcdef}{a}|
\exemple*|\StrBehind{abcdef}{z}|
\exemple*|\StrBehind{a b c d}{c}|
\exemple*|\StrBehind{a b c d}{ }|
\exemple*|\StrBehind[2]{a b c d}{ }|
\exemple*|\StrBehind[3]{a b c d}{ }|
\exemple*|\StrBehind[9]{a b c d}{ }|
\exemple*|\StrBehind[-7]{a b c d}{ }|
\exemple*|\StrBehind{abcdef}{Z}|
\exemple|\StrBehind[1]{aaaaaa}{aa}|
\exemple|\StrBehind[2]{aaaaaa}{aa}|
\exemple*|\StrBehind[3]{aaaaaa}{aa}|
\exemple*|\StrBehind[4]{aaaaaa}{aa}|
\exemple*|\StrBehind{a}{}|
\exemple*|\StrBehind{}{a}|
\exemple*|\StrBehind{}{}|

\AvecArgOptionnel
\exemple|\StrBehind{abcedef}{e}[\aa]\aa|
\exemple*|\StrBehind{abcdef}{a}[\aa]\aa|
\exemple*|\StrBehind{abcdef}{z}[\aa]\aa|
\exemple*|\StrBehind{a b c d}{c}[\aa]\aa|
\exemple*|\StrBehind{a b c d}{ }[\aa]\aa|
\exemple*|\StrBehind[2]{a b c d}{ }[\aa]\aa|
\exemple*|\StrBehind[3]{a b c d}{ }[\aa]\aa|
\exemple*|\StrBehind[9]{a b c d}{ }[\aa]\aa|
\exemple*|\StrBehind[-7]{a b c d}{ }[\aa]\aa|
\exemple*|\StrBehind{abcdef}{Z}[\aa]\aa|
\exemple|\StrBehind[1]{aaaaaa}{aa}[\aa]\aa|
\exemple|\StrBehind[2]{aaaaaa}{aa}[\aa]\aa|
\exemple*|\StrBehind[3]{aaaaaa}{aa}[\aa]\aa|
\exemple*|\StrBehind[4]{aaaaaa}{aa}[\aa]\aa|
\exemple*|\StrBehind{a}{}[\aa]\aa|
\exemple*|\StrBehind{}{a}[\aa]\aa|
\exemple*|\StrBehind{}{}[\aa]\aa|

\chapitre{La macro}{StrBetween}

\exemple|\StrBetween{abcdef}{b}{e}|
\exemple*|\StrBetween{aZaaaaZa}{Z}{Z}|
\exemple*|\StrBetween[1,2]{aZaaaaZa}{Z}{Z}|
\exemple*|\StrBetween{a b c d}{a}{c}|
\exemple*|\StrBetween{a b c d}{a }{ d}|
\exemple*|\StrBetween{abcdef}{a}{Z}|
\exemple*|\StrBetween{abcdef}{Y}{Z}|
\exemple*|\StrBetween[2,5]{aAaBaCaDa}{a}{a}|
\exemple*|\StrBetween[4,1]{ab1ab2ab3ab4ab}{b}{a}|
\exemple*|\StrBetween[3,4]{a b c d e f}{ }{ }|
\exemple|\StrBetween[1,3]{aaaaaa}{aa}{aa}|
\exemple*|\StrBetween{abcdef}{a}{}|
\exemple*|\StrBetween{abcdef}{}{f}|
\exemple*|\StrBetween{}{a}{b}|

\AvecArgOptionnel
\exemple|\StrBetween{abcdef}{b}{e}[\aa]\aa|
\exemple*|\StrBetween{aZaaaaZa}{Z}{Z}[\aa]\aa|
\exemple*|\StrBetween[1,2]{aZaaaaZa}{Z}{Z}[\aa]\aa|
\exemple*|\StrBetween{a b c d}{a}{c}[\aa]\aa|
\exemple*|\StrBetween{a b c d}{a }{ d}[\aa]\aa|
\exemple*|\StrBetween{abcdef}{a}{Z}[\aa]\aa|
\exemple*|\StrBetween{abcdef}{Y}{Z}[\aa]\aa|
\exemple*|\StrBetween[2,5]{aAaBaCaDa}{a}{a}[\aa]\aa|
\exemple*|\StrBetween[4,1]{ab1ab2ab3ab4ab}{b}{a}[\aa]\aa|
\exemple*|\StrBetween[3,4]{a b c d e f}{ }{ }[\aa]\aa|
\exemple|\StrBetween[1,3]{aaaaaa}{aa}{aa}[\aa]\aa|
\exemple*|\StrBetween{abcdef}{a}{}[\aa]\aa|
\exemple*|\StrBetween{abcdef}{}{f}[\aa]\aa|
\exemple*|\StrBetween{}{a}{b}[\aa]\aa|

\chapitre{La macro}{StrSubstitute}

\exemple|\StrSubstitute{abcdef}{c}{ZZ}|
\exemple|\StrSubstitute{aaaaaaa}{aa}{w}|
\exemple|\StrSubstitute[0]{abacada}{a}{.}|
\exemple|\StrSubstitute[1]{abacada}{a}{.}|
\exemple|\StrSubstitute[2]{abacada}{a}{.}|
\exemple|\StrSubstitute[3]{abacada}{a}{.}|
\exemple|\StrSubstitute[4]{abacada}{a}{.}|
\exemple|\StrSubstitute[5]{abacada}{a}{.}|
\exemple|\StrSubstitute{a b c d e}{ }{,}|
\exemple|\StrSubstitute{a b c d e}{ }{}|
\exemple|\StrSubstitute{abcdef}{}{A}|
\exemple|\StrSubstitute{abcdef}{}{}|
\exemple*|\StrSubstitute{}{a}{b}|
\exemple*|\StrSubstitute{}{}{}|

\AvecArgOptionnel
\exemple|\StrSubstitute{abcdef}{c}{ZZ}[\aa]\aa|
\exemple|\StrSubstitute{aaaaaaa}{aa}{w}[\aa]\aa|
\exemple|\StrSubstitute[0]{abacada}{a}{.}[\aa]\aa|
\exemple|\StrSubstitute[1]{abacada}{a}{.}[\aa]\aa|
\exemple|\StrSubstitute[2]{abacada}{a}{.}[\aa]\aa|
\exemple|\StrSubstitute[3]{abacada}{a}{.}[\aa]\aa|
\exemple|\StrSubstitute[4]{abacada}{a}{.}[\aa]\aa|
\exemple|\StrSubstitute[5]{abacada}{a}{.}[\aa]\aa|
\exemple|\StrSubstitute{a b c d e}{ }{,}[\aa]\aa|
\exemple|\StrSubstitute{a b c d e}{ }{}[\aa]\aa|
\exemple|\StrSubstitute{abcdef}{}{A}[\aa]\aa|
\exemple|\StrSubstitute{abcdef}{}{}[\aa]\aa|
\exemple*|\StrSubstitute{}{a}{b}[\aa]\aa|
\exemple*|\StrSubstitute{}{}{}[\aa]\aa|

\chapitre{La macro}{StrDel}

\exemple|\StrDel{a1a2a3a4}{a}|
\exemple|\StrDel[2]{a1a2a3a4}{a}|
\exemple|\StrDel[-2]{a1a2a3a4}{a}|
\exemple|\StrDel[10]{a1a2a3a4}{a}|
\exemple|\StrDel[3]{a b c d e}{a}|

\AvecArgOptionnel
\exemple|\StrDel{a1a2a3a4}{a}[\aa]\aa|
\exemple|\StrDel[2]{a1a2a3a4}{a}[\aa]\aa|
\exemple|\StrDel[-2]{a1a2a3a4}{a}[\aa]\aa|
\exemple|\StrDel[10]{a1a2a3a4}{a}[\aa]\aa|
\exemple|\StrDel[3]{a b c d e}{a}[\aa]\aa|

\chapitre{La macro}{StrLen}


\exemple|\StrLen{abcdef}|
\exemple|\StrLen{a b c}|
\exemple|\StrLen{ a b c }|
\exemple|\StrLen{a}|
\exemple|\StrLen{}|

\AvecArgOptionnel
\exemple|\StrLen{abcdef}[\aa]\aa|
\exemple|\StrLen{a b c}[\aa]\aa|
\exemple|\StrLen{ a b c }[\aa]\aa|
\exemple|\StrLen{a}[\aa]\aa|
\exemple|\StrLen{}[\aa]\aa|

\chapitre{la macro}{StrMid}

\exemple|\StrMid{abcdef}{2}{5}|
\exemple*|\StrMid{a b c d}{2}{6}|
\exemple*|\StrMid{abcdef}{4}{2}|
\exemple|\StrMid{abcdef}{-4}{3}|
\exemple*|\StrMid{abcdef}{-4}{-1}|
\exemple|\StrMid{abcdef}{-4}{20}|
\exemple*|\StrMid{abcdef}{8}{10}|
\exemple|\StrMid{abcdef}{2}{2}|
\exemple|\StrMid{aaaaaa}{3}{6}|
\exemple*|\StrMid{}{4}{5}|

\AvecArgOptionnel
\exemple|\StrMid{abcdef}{2}{5}[\aa]\aa|
\exemple*|\StrMid{a b c d}{2}{6}[\aa]\aa|
\exemple*|\StrMid{abcdef}{4}{2}[\aa]\aa|
\exemple|\StrMid{abcdef}{-4}{3}[\aa]\aa|
\exemple*|\StrMid{abcdef}{-4}{-1}[\aa]\aa|
\exemple|\StrMid{abcdef}{-4}{20}[\aa]\aa|
\exemple*|\StrMid{abcdef}{8}{10}[\aa]\aa|
\exemple|\StrMid{abcdef}{2}{2}[\aa]\aa|
\exemple|\StrMid{aaaaaa}{3}{6}[\aa]\aa|
\exemple*|\StrMid{}{4}{5}[\aa]\aa|

\chapitre{La macro}{StrGobbleLeft}

\exemple|\StrGobbleLeft{abcdef}{3}|
\exemple*|\StrGobbleLeft{a b c d}{3}|
\exemple|\StrGobbleLeft{abcdef}{-3}|
\exemple*|\StrGobbleLeft{abcdef}{9}|
\exemple|\StrGobbleLeft{aaaaa}{4}|
\exemple*|\StrGobbleLeft{}{2}|

\AvecArgOptionnel
\exemple|\StrGobbleLeft{abcdef}{3}[\aa]\aa|
\exemple*|\StrGobbleLeft{a b c d}{3}[\aa]\aa|
\exemple|\StrGobbleLeft{abcdef}{-3}[\aa]\aa|
\exemple*|\StrGobbleLeft{abcdef}{9}[\aa]\aa|
\exemple|\StrGobbleLeft{aaaaa}{4}[\aa]\aa|
\exemple*|\StrGobbleLeft{}{2}[\aa]\aa|

\chapitre{La macro}{StrGobbleRight}

\exemple|\StrGobbleRight{abcdef}{3}|
\exemple*|\StrGobbleRight{a b c d}{3}|
\exemple|\StrGobbleRight{abcdef}{-3}|
\exemple*|\StrGobbleRight{abcdef}{9}|
\exemple|\StrGobbleRight{aaaaa}{4}|
\exemple*|\StrGobbleRight{}{2}|

\AvecArgOptionnel
\exemple|\StrGobbleRight{abcdef}{3}[\aa]\aa|
\exemple*|\StrGobbleRight{a b c d}{3}[\aa]\aa|
\exemple|\StrGobbleRight{abcdef}{-3}[\aa]\aa|
\exemple*|\StrGobbleRight{abcdef}{9}[\aa]\aa|
\exemple|\StrGobbleRight{aaaaa}{4}[\aa]\aa|
\exemple*|\StrGobbleRight{}{2}[\aa]\aa|

\chapitre{La macro}{StrLeft}

\exemple|\StrLeft{abcdef}{3}|
\exemple*|\StrLeft{a b c d}{3}|
\exemple*|\StrLeft{abcdef}{-3}|
\exemple*|\StrLeft{abcdef}{9}|
\exemple|\StrLeft{aaaaa}{4}|
\exemple*|\StrLeft{}{2}|

\AvecArgOptionnel
\exemple|\StrLeft{abcdef}{3}[\aa]\aa|
\exemple*|\StrLeft{a b c d}{3}[\aa]\aa|
\exemple*|\StrLeft{abcdef}{-3}[\aa]\aa|
\exemple*|\StrLeft{abcdef}{9}[\aa]\aa|
\exemple|\StrLeft{aaaaa}{4}[\aa]\aa|
\exemple*|\StrLeft{}{2}[\aa]\aa|

\chapitre{La macro}{StrRight}

\exemple|\StrRight{abcdef}{3}|
\exemple*|\StrRight{a b c d}{3}|
\exemple*|\StrRight{abcdef}{-3}|
\exemple*|\StrRight{abcdef}{9}|
\exemple|\StrRight{aaaaa}{4}|
\exemple*|\StrRight{}{2}|

\AvecArgOptionnel
\exemple|\StrRight{abcdef}{3}[\aa]\aa|
\exemple*|\StrRight{a b c d}{3}[\aa]\aa|
\exemple*|\StrRight{abcdef}{-3}[\aa]\aa|
\exemple*|\StrRight{abcdef}{9}[\aa]\aa|
\exemple|\StrRight{aaaaa}{4}[\aa]\aa|
\exemple*|\StrRight{}{2}[\aa]\aa|

\chapitre{la macro}{StrChar}

\exemple|\StrChar{abcdef}{5}|
\exemple*|\StrChar{a b c d}{4}|
\exemple|\StrChar{a b c d}{7}|
\exemple*|\StrChar{abcdef}{10}|
\exemple*|\StrChar{abcdef}{-5}|
\exemple*|\StrChar{}{3}|

\AvecArgOptionnel
\exemple|\StrChar{abcdef}{5}[\aa]\aa|
\exemple*|\StrChar{a b c d}{4}[\aa]\aa|
\exemple|\StrChar{a b c d}{7}[\aa]\aa|
\exemple*|\StrChar{abcdef}{10}[\aa]\aa|
\exemple*|\StrChar{abcdef}{-5}[\aa]\aa|
\exemple*|\StrChar{}{3}[\aa]\aa|

\chapitre{La macro}{StrCount}

\exemple|\StrCount{abcdef}{d}|
\exemple|\StrCount{a b c d}{ }|
\exemple|\StrCount{aaaaaa}{aa}|
\exemple|\StrCount{abcdef}{Z}|
\exemple|\StrCount{abcdef}{}|
\exemple|\StrCount{}{a}|
\exemple|\StrCount{}{}|

\AvecArgOptionnel
\exemple|\StrCount{abcdef}{d}[\aa]\aa|
\exemple|\StrCount{a b c d}{ }[\aa]\aa|
\exemple|\StrCount{aaaaaa}{aa}[\aa]\aa|
\exemple|\StrCount{abcdef}{Z}[\aa]\aa|
\exemple|\StrCount{abcdef}{}[\aa]\aa|
\exemple|\StrCount{}{a}[\aa]\aa|
\exemple|\StrCount{}{}[\aa]\aa|

\chapitre{La macro}{StrPosition}

\exemple|\StrPosition{abcdef}{c}|
\exemple|\StrPosition{abcdef}{Z}|
\exemple|\StrPosition{a b c d}{ }|
\exemple|\StrPosition[3]{a b c d}{ }|
\exemple|\StrPosition[8]{a b c d}{ }|
\exemple|\StrPosition{aaaaaa}{aa}|
\exemple|\StrPosition[2]{aaaaaa}{aa}|
\exemple|\StrPosition[3]{aaaaaa}{aa}|
\exemple|\StrPosition{abcdef}{}|
\exemple|\StrPosition{}{a}|
\exemple|\StrPosition{}{}|

\AvecArgOptionnel
\exemple|\StrPosition{abcdef}{c}[\aa]\aa|
\exemple|\StrPosition{abcdef}{Z}[\aa]\aa|
\exemple|\StrPosition{a b c d}{ }[\aa]\aa|
\exemple|\StrPosition[3]{a b c d}{ }[\aa]\aa|
\exemple|\StrPosition[8]{a b c d}{ }[\aa]\aa|
\exemple|\StrPosition{aaaaaa}{aa}[\aa]\aa|
\exemple|\StrPosition[2]{aaaaaa}{aa}[\aa]\aa|
\exemple|\StrPosition[3]{aaaaaa}{aa}[\aa]\aa|
\exemple|\StrPosition{abcdef}{}[\aa]\aa|
\exemple|\StrPosition{}{a}[\aa]\aa|
\exemple|\StrPosition{}{}[\aa]\aa|

\chapitre{La macro}{StrCompare}

La tolérance normale :\par
\exemple|\StrCompare{abcdefghij}{abc}|
\exemple|\StrCompare{A}{A}|
\exemple|\StrCompare{abcdef}{a bd}|
\exemple|\StrCompare{ }{ }|
\exemple|\StrCompare{}{abcd}|
\exemple|\StrCompare{abcd}{}|
\exemple|\StrCompare{123456}{1234}|
\exemple|\StrCompare{a b c d}{a bcd}|
\exemple|\StrCompare{}{}|
\exemple|\StrCompare{eee}{eeee}|
\exemple|\StrCompare{eeee}{eee}|
\exemple|\StrCompare{totutu}{tututu}|
\exemple|\StrCompare{abcd}{abyz}|

\AvecArgOptionnel
\exemple|\StrCompare{abcdefghij}{abc}[\aa]\aa|
\exemple|\StrCompare{A}{A}[\aa]\aa|
\exemple|\StrCompare{abcdef}{a bd}[\aa]\aa|
\exemple|\StrCompare{ }{ }[\aa]\aa|
\exemple|\StrCompare{}{abcd}[\aa]\aa|
\exemple|\StrCompare{abcd}{}[\aa]\aa|
\exemple|\StrCompare{123456}{1234}[\aa]\aa|
\exemple|\StrCompare{a b c d}{a bcd}[\aa]\aa|
\exemple|\StrCompare{}{}[\aa]\aa|
\exemple|\StrCompare{eee}{eeee}[\aa]\aa|
\exemple|\StrCompare{eeee}{eee}[\aa]\aa|
\exemple|\StrCompare{totutu}{tututu}[\aa]\aa|
\exemple|\StrCompare{abcd}{abyz}[\aa]\aa|

La tolérance stricte :\par\comparestrict
\exemple|\StrCompare{abcdefghij}{abc}|
\exemple|\StrCompare{A}{A}|
\exemple|\StrCompare{abcdef}{a bd}|
\exemple|\StrCompare{ }{ }|
\exemple|\StrCompare{}{abcd}|
\exemple|\StrCompare{abcd}{}|
\exemple|\StrCompare{123456}{1234}|
\exemple|\StrCompare{a b c d}{a bcd}|
\exemple|\StrCompare{}{}|
\exemple|\StrCompare{eee}{eeee}|
\exemple|\StrCompare{eeee}{eee}|
\exemple|\StrCompare{totutu}{tututu}|
\exemple|\StrCompare{abcd}{abyz}|

\AvecArgOptionnel
\exemple|\StrCompare{abcdefghij}{abc}[\aa]\aa|
\exemple|\StrCompare{A}{A}[\aa]\aa|
\exemple|\StrCompare{abcdef}{a bd}[\aa]\aa|
\exemple|\StrCompare{ }{ }[\aa]\aa|
\exemple|\StrCompare{}{abcd}[\aa]\aa|
\exemple|\StrCompare{abcd}{}[\aa]\aa|
\exemple|\StrCompare{123456}{1234}[\aa]\aa|
\exemple|\StrCompare{a b c d}{a bcd}[\aa]\aa|
\exemple|\StrCompare{}{}[\aa]\aa|
\exemple|\StrCompare{eee}{eeee}[\aa]\aa|
\exemple|\StrCompare{eeee}{eee}[\aa]\aa|
\exemple|\StrCompare{totutu}{tututu}[\aa]\aa|
\exemple|\StrCompare{abcd}{abyz}[\aa]\aa|
\vskip5em

\hfill{\hugerm Le mode \hugett\string\noexpandarg}\hfill{}

\vskip-1ex\hfil\hbox to8cm{\hrulefill}\hfil{}\vskip3.5ex

Dans toute la suite sauf si c'est précisé, la commande {\tt\string\noexpandarg} est activée.\vskip1.5ex

\catcode`\@=11\relax
\expandafter\long\expandafter\def\csname xs_assign_verb\endcsname#1{%
	\tokenize\cs@resultat{#1}%
	\leavevmode\hbox to0.7\hsize{\hfil\tt#1}\quad\frontiere\cs@resultat\frontiere\hfil\par}%
\catcode`\@=12\relax
\noexpandarg

\chapitre{Le test}{IfSubStr}

\exemple|\noexploregroups|
\exemple|\IfSubStr{1$2$\a{34}\bc5}{2}{vrai}{faux}|
\exemple|\IfSubStr{1$2$\a{34}\bc5}{34}{vrai}{faux}|
\exemple|\IfSubStr{1$2$\a{34}\bc5}{{34}}{vrai}{faux}|
\exemple|\IfSubStr{1$2$\a{34}\bc5}{\b}{vrai}{faux}|
\exemple|\IfSubStr{1$2$\a{34}\bc5}{\bc}{vrai}{faux}|
\exemple|\IfSubStr{1$2$\a{34}\bc5}{\bc5}{vrai}{faux}|
\exemple|\IfSubStr{1$2$\a{34}\bc5}{\bc{5}}{vrai}{faux}|
\exemple|\IfSubStr[1]{\a1{\a1{\a1}\a2}\a3}{\a}{vrai}{faux}|
\exemple|\IfSubStr[2]{\a1{\a1{\a1}\a2}\a3}{\a}{vrai}{faux}|
\exemple|\IfSubStr[3]{\a1{\a1{\a1}\a2}\a3}{\a}{vrai}{faux}|
\exemple|\IfSubStr[4]{\a1{\a1{\a1}\a2}\a3}{\a}{vrai}{faux}|
\exemple|\exploregroups|
\exemple|\IfSubStr{1$2$\a{34}\bc5}{2}{vrai}{faux}|
\exemple|\IfSubStr{1$2$\a{34}\bc5}{34}{vrai}{faux}|
\exemple|\IfSubStr{1$2$\a{34}\bc5}{{34}}{vrai}{faux}|
\exemple|\IfSubStr{1$2$\a{34}\bc5}{\b}{vrai}{faux}|
\exemple|\IfSubStr{1$2$\a{34}\bc5}{\bc}{vrai}{faux}|
\exemple|\IfSubStr{1$2$\a{34}\bc5}{\bc5}{vrai}{faux}|
\exemple|\IfSubStr{1$2$\a{34}\bc5}{\bc{5}}{vrai}{faux}|
\exemple|\IfSubStr[1]{\a1{\a1{\a1}\a2}\a3}{\a}{vrai}{faux}|
\exemple|\IfSubStr[2]{\a1{\a1{\a1}\a2}\a3}{\a}{vrai}{faux}|
\exemple|\IfSubStr[3]{\a1{\a1{\a1}\a2}\a3}{\a}{vrai}{faux}|
\exemple|\IfSubStr[4]{\a1{\a1{\a1}\a2}\a3}{\a}{vrai}{faux}|

\chapitre{Le test}{IfBeginWith}

Les tests doivent donner des résultats identiques ci-dessous puisque {\tt\string\IfBeginWith} est indifférent au mode d'exploration des groupes !\vskip0.7ex

\exemple|\noexploregroups|
\exemple|\IfBeginWith{{\a}123\b456}{\a}{vrai}{faux}|
\exemple|\IfBeginWith{{\a}123\b456}{{\a}}{vrai}{faux}|
\exemple|\IfBeginWith{{\a1}\b\c\d}{\a}{vrai}{faux}|
\exemple|\IfBeginWith{{1}23456}{12}{vrai}{faux}|
\exemple|\IfBeginWith{{1}23456}{1}{vrai}{faux}|
\exemple|\IfBeginWith{{1}23456}{{1}2}{vrai}{faux}|
\exemple|\exploregroups|
\exemple|\IfBeginWith{{\a}123\b456}{\a}{vrai}{faux}|
\exemple|\IfBeginWith{{\a}123\b456}{{\a}}{vrai}{faux}|
\exemple|\IfBeginWith{{\a1}\b\c\d}{\a}{vrai}{faux}|
\exemple|\IfBeginWith{{1}23456}{12}{vrai}{faux}|
\exemple|\IfBeginWith{{1}23456}{1}{vrai}{faux}|
\exemple|\IfBeginWith{{1}23456}{{1}2}{vrai}{faux}|

\chapitre{Le test}{IfEndWith}

Les tests doivent donner des résultats identiques ci-dessous puisque {\tt\string\IfEndWith} est indifférent au mode d'exploration des groupes !\vskip0.7ex

\exemple|\noexploregroups|
\exemple|\IfEndWith{\a1\b2{\c3}}{\c3}{vrai}{faux}|
\exemple|\IfEndWith{\a1\b2{\c3}}{{\c3}}{vrai}{faux}|
\exemple|\IfEndWith{\a1\b2{\c3}}{3}{vrai}{faux}|
\exemple|\IfEndWith{12345{6}}{56}{vrai}{faux}|
\exemple|\IfEndWith{12345{6}}{6}{vrai}{faux}|
\exemple|\IfEndWith{12345{6}}{5{6}}{vrai}{faux}|
\exemple|\exploregroups|
\exemple|\IfEndWith{\a1\b2{\c3}}{\c3}{vrai}{faux}|
\exemple|\IfEndWith{\a1\b2{\c3}}{{\c3}}{vrai}{faux}|
\exemple|\IfEndWith{\a1\b2{\c3}}{3}{vrai}{faux}|
\exemple|\IfEndWith{12345{6}}{56}{vrai}{faux}|
\exemple|\IfEndWith{12345{6}}{6}{vrai}{faux}|
\exemple|\IfEndWith{12345{6}}{5{6}}{vrai}{faux}|

\chapitre{Le test}{IfSubStrBefore}

\exemple|\noexploregroups|
\exemple|\IfSubStrBefore[1,1]{\a1\a2\a3\b1\b2\b3}{2}{\b}{vrai}{faux}|
\exemple|\IfSubStrBefore[2,1]{\a1\a2\a3\b1\b2\b3}{2}{\b}{vrai}{faux}|
\exemple|\IfSubStrBefore[2,3]{\a1\a2\a3\b1\b2\b3}{\a}{\b}{vrai}{faux}|
\exemple|\IfSubStrBefore[1,1]{\a1{\a2\a3\b1}\b2\b3}{2}{\b}{vrai}{faux}|
\exemple|\IfSubStrBefore[1,2]{\a1{\a2\a3\b1}\b2\b3}{3}{\b}{vrai}{faux}|
\exemple|\exploregroups|
\exemple|\IfSubStrBefore[1,1]{\a1\a2\a3\b1\b2\b3}{2}{\b}{vrai}{faux}|
\exemple|\IfSubStrBefore[2,1]{\a1\a2\a3\b1\b2\b3}{2}{\b}{vrai}{faux}|
\exemple|\IfSubStrBefore[2,3]{\a1\a2\a3\b1\b2\b3}{\a}{\b}{vrai}{faux}|
\exemple|\IfSubStrBefore[1,1]{\a1{\a2\a3\b1}\b2\b3}{2}{\b}{vrai}{faux}|
\exemple|\IfSubStrBefore[1,2]{\a1{\a2\a3\b1}\b2\b3}{3}{\b}{vrai}{faux}|

\chapitre{Le test}{IfStrBehind}

\exemple|\noexploregroups|
\exemple|\IfSubStrBehind[2,1]{\a1\a2\a3\b1\b2\b3}{2}{\b}{vrai}{faux}|
\exemple|\IfSubStrBehind[3,1]{\a1\a2\a3\b1\b2\b3}{\a}{\b}{vrai}{faux}|
\exemple|\IfSubStrBehind[1,1]{\a1\a2\a3\b1\b2\b3}{\b}{3}{vrai}{faux}|
\exemple|\IfSubStrBehind[2,1]{\a1{\a2\a3\b1}\b2\b3}{\b}{3}{vrai}{faux}|
\exemple|\IfSubStrBehind[1,1]{\a1{\a2\a3\b1}\b2\b3}{3}{\b}{vrai}{faux}|
\exemple|\exploregroups|
\exemple|\IfSubStrBehind[2,1]{\a1\a2\a3\b1\b2\b3}{2}{\b}{vrai}{faux}|
\exemple|\IfSubStrBehind[3,1]{\a1\a2\a3\b1\b2\b3}{\a}{\b}{vrai}{faux}|
\exemple|\IfSubStrBehind[1,1]{\a1\a2\a3\b1\b2\b3}{\b}{3}{vrai}{faux}|
\exemple|\IfSubStrBehind[2,1]{\a1{\a2\a3\b1}\b2\b3}{\b}{3}{vrai}{faux}|
\exemple|\IfSubStrBehind[1,1]{\a1{\a2\a3\b1}\b2\b3}{3}{\b}{vrai}{faux}|

\chapitre{Le test}{IfInteger}

Dans les exemples ci-dessous, on examine la différence de comportement de la macro {\tt\string\IfInteger} selon les modes de développement des arguments.\vskip0.7ex

\exemple|\def\nbA{-12}\def\nbB{498}|
\exemple|\def\nbAA{\nbA}\def\nbBB{\nbB}|\vskip0.7ex
\exemple|\fullexpandarg|
\exemple|\IfInteger{\nbA}{vrai}{faux}|
\exemple|\IfInteger{\nbA5\nbA}{vrai}{faux}|
\exemple|\IfInteger{\nbA6\nbB}{vrai}{faux}|
\exemple|\IfInteger{\nbAA7\nbBB}{vrai}{faux}|\vskip0.7ex
\exemple|\expandarg|
\exemple|\IfInteger{\nbA}{vrai}{faux}|
\exemple|\IfInteger{\nbA5\nbA}{vrai}{faux}|
\exemple|\IfInteger{\nbA6\nbB}{vrai}{faux}|
\exemple|\IfInteger{\nbAA7\nbBB}{vrai}{faux}|\vskip0.7ex
\exemple|\noexpandarg|
\exemple|\IfInteger{\nbA}{vrai}{faux}|
\exemple|\IfInteger{\nbA5\nbA}{vrai}{faux}|
\exemple|\IfInteger{\nbA6\nbB}{vrai}{faux}|
\exemple|\IfInteger{\nbAA7\nbBB}{vrai}{faux}|

\chapitre{Le test}{IfDecimal}

Dans les exemples ci-dessous, on examine la différence de comportement de la macro {\tt\string\IfDecimal} selon les modes de développement des arguments.\vskip0.7ex

\exemple|\def\nbA{-12}\def\nbB{498}|
\exemple|\def\nbAA{\nbA}\def\nbBB{\nbB}|\vskip0.7ex
\exemple|\fullexpandarg|
\exemple|\IfDecimal{\nbA,\nbB}{vrai}{faux}|
\exemple|\IfDecimal{\nbAA.\nbB}{vrai}{faux}|
\exemple|\IfDecimal{\nbB,777}{vrai}{faux}|
\exemple|\IfDecimal{3\nbB,777}{vrai}{faux}|
\exemple|\IfDecimal{\nbB,\nbB}{vrai}{faux}|\vskip0.7ex
\exemple|\expandarg|
\exemple|\IfDecimal{\nbA,\nbB}{vrai}{faux}|
\exemple|\IfDecimal{\nbAA.\nbB}{vrai}{faux}|
\exemple|\IfDecimal{\nbB,777}{vrai}{faux}|
\exemple|\IfDecimal{3\nbB,777}{vrai}{faux}|
\exemple|\IfDecimal{\nbB,\nbB}{vrai}{faux}|\vskip0.7ex
\exemple|\noexpandarg|
\exemple|\IfDecimal{\nbA,\nbB}{vrai}{faux}|
\exemple|\IfDecimal{\nbAA.\nbB}{vrai}{faux}|
\exemple|\IfDecimal{\nbB,777}{vrai}{faux}|
\exemple|\IfDecimal{3\nbB,777}{vrai}{faux}|
\exemple|\IfDecimal{\nbB,\nbB}{vrai}{faux}|

\chapitre{La macro}{StrBefore}

\exemple|\noexploregroups|
\exemple|\StrBefore[2]{1\a2\a3{4\a5{6\a7}8\a}9\a0}{\a}[\cmd]|
\exemple|\detokenize\expandafter{\cmd}|\vskip0.7ex
\exemple|\StrBefore[3]{1\a2\a3{4\a5{6\a7}8\a}9\a0}{\a}[\cmd]|
\exemple|\detokenize\expandafter{\cmd}|\vskip0.7ex
\exemple|\StrBefore[4]{1\a2\a3{4\a5{6\a7}8\a}9\a0}{\a}[\cmd]|
\exemple|\detokenize\expandafter{\cmd}|\vskip0.7ex
\exemple|\StrBefore[5]{1\a2\a3{4\a5{6\a7}8\a}9\a0}{\a}[\cmd]|
\exemple|\detokenize\expandafter{\cmd}|\vskip0.7ex
\exemple|\StrBefore[6]{1\a2\a3{4\a5{6\a7}8\a}9\a0}{\a}[\cmd]|
\exemple|\detokenize\expandafter{\cmd}|\vskip0.7ex
\exemple|\exploregroups|
\exemple|\StrBefore[2]{1\a2\a3{4\a5{6\a7}8\a}9\a0}{\a}[\cmd]|
\exemple|\detokenize\expandafter{\cmd}|\vskip0.7ex
\exemple|\StrBefore[3]{1\a2\a3{4\a5{6\a7}8\a}9\a0}{\a}[\cmd]|
\exemple|\detokenize\expandafter{\cmd}|\vskip0.7ex
\exemple|\StrBefore[4]{1\a2\a3{4\a5{6\a7}8\a}9\a0}{\a}[\cmd]|
\exemple|\detokenize\expandafter{\cmd}|\vskip0.7ex
\exemple|\StrBefore[5]{1\a2\a3{4\a5{6\a7}8\a}9\a0}{\a}[\cmd]|
\exemple|\detokenize\expandafter{\cmd}|\vskip0.7ex
\exemple|\StrBefore[6]{1\a2\a3{4\a5{6\a7}8\a}9\a0}{\a}[\cmd]|
\exemple|\detokenize\expandafter{\cmd}|

\chapitre{La macro}{StrBehind}

\exemple|\noexploregroups|
\exemple|\StrBehind[2]{1\a2\a3{4\a5{6\a7}8\a}9\a0}{\a}[\cmd]|
\exemple|\detokenize\expandafter{\cmd}|\vskip0.7ex
\exemple|\StrBehind[3]{1\a2\a3{4\a5{6\a7}8\a}9\a0}{\a}[\cmd]|
\exemple|\detokenize\expandafter{\cmd}|\vskip0.7ex
\exemple|\StrBehind[4]{1\a2\a3{4\a5{6\a7}8\a}9\a0}{\a}[\cmd]|
\exemple|\detokenize\expandafter{\cmd}|\vskip0.7ex
\exemple|\StrBehind[5]{1\a2\a3{4\a5{6\a7}8\a}9\a0}{\a}[\cmd]|
\exemple|\detokenize\expandafter{\cmd}|\vskip0.7ex
\exemple|\StrBehind[6]{1\a2\a3{4\a5{6\a7}8\a}9\a0}{\a}[\cmd]|
\exemple|\detokenize\expandafter{\cmd}|\vskip0.7ex
\exemple|\exploregroups|
\exemple|\StrBehind[2]{1\a2\a3{4\a5{6\a7}8\a}9\a0}{\a}[\cmd]|
\exemple|\detokenize\expandafter{\cmd}|\vskip0.7ex
\exemple|\StrBehind[3]{1\a2\a3{4\a5{6\a7}8\a}9\a0}{\a}[\cmd]|
\exemple|\detokenize\expandafter{\cmd}|\vskip0.7ex
\exemple|\StrBehind[4]{1\a2\a3{4\a5{6\a7}8\a}9\a0}{\a}[\cmd]|
\exemple|\detokenize\expandafter{\cmd}|\vskip0.7ex
\exemple|\StrBehind[5]{1\a2\a3{4\a5{6\a7}8\a}9\a0}{\a}[\cmd]|
\exemple|\detokenize\expandafter{\cmd}|\vskip0.7ex
\exemple|\StrBehind[6]{1\a2\a3{4\a5{6\a7}8\a}9\a0}{\a}[\cmd]|
\exemple|\detokenize\expandafter{\cmd}|

\chapitre{La macro}{StrBetween}

La commande {\tt\string\StrBetween} opère en mode {\tt\string\noexploregroups}, quelque soit le mode d'exploration en cours.\vskip0.7ex

\exemple|\StrBetween[1,3]{\a1\a2{3\a4}5\a6{7\a8}9\a0}{2}{\a}[\cmd]|
\exemple|\detokenize\expandafter{\cmd}|\vskip0.7ex
\exemple|\StrBetween[2,3]{\a1\a2{3\a4}5\a6{7\a8}9\a0}{\a}{\a}[\cmd]|
\exemple|\detokenize\expandafter{\cmd}|\vskip0.7ex
\exemple|\StrBetween[1,3]{\a1\a2{3\a4}5\a6{7\a8}9\a0}{3}{\a}[\cmd]|
\exemple|\detokenize\expandafter{\cmd}|\vskip0.7ex
\exemple|\StrBetween[2,4]{\a1\a2{3\a4}5\a6{7\a8}9\a0}{\a}{\a}[\cmd]|
\exemple|\detokenize\expandafter{\cmd}|\vskip0.7ex

\chapitre{La macro}{StrSubstitute}

\exemple|\noexploregroups|
\exemple|\StrSubstitute{\a1{2\a{3\a}4\a}\a5\a}{\a}{\X}[\cmd]|
\exemple|\detokenize\expandafter{\cmd}|\vskip0.7ex
\exemple|\StrSubstitute[2]{\a1{2\a{3\a}4\a}\a5\a}{\a}{\X}[\cmd]|
\exemple|\detokenize\expandafter{\cmd}|\vskip0.7ex
\exemple|\StrSubstitute{\a1{2\a{3\a}4\a}\a5\a}{2}{X}[\cmd]|
\exemple|\detokenize\expandafter{\cmd}|\vskip0.7ex
\exemple|\StrSubstitute{\a1{2\a{3\a}4\a}\a5\a}{{3\a}}{XXX}[\cmd]|
\exemple|\detokenize\expandafter{\cmd}|\vskip0.7ex
\exemple|\StrSubstitute{\a1{2\a{3\a}4\a}\a5\a}{3\a}{XXX}[\cmd]|
\exemple|\detokenize\expandafter{\cmd}|\vskip0.7ex
\exemple|\StrSubstitute{a1{b1\bgroup c1}\egroup d1}{1}{X}[\cmd]|
\exemple|\detokenize\expandafter{\cmd}|\smallskip
\exemple|\exploregroups|
\exemple|\StrSubstitute{\a1{2\a{3\a}4\a}\a5\a}{\a}{\X}[\cmd]|
\exemple|\detokenize\expandafter{\cmd}|\vskip0.7ex
\exemple|\StrSubstitute[2]{\a1{2\a{3\a}4\a}\a5\a}{\a}{\X}[\cmd]|
\exemple|\detokenize\expandafter{\cmd}|\vskip0.7ex
\exemple|\StrSubstitute{\a1{2\a{3\a}4\a}\a5\a}{2}{X}[\cmd]|
\exemple|\detokenize\expandafter{\cmd}|\vskip0.7ex
\exemple|\StrSubstitute{\a1{2\a{3\a}4\a}\a5\a}{{3\a}}{XXX}[\cmd]|
\exemple|\detokenize\expandafter{\cmd}|\vskip0.7ex
\exemple|\StrSubstitute{\a1{2\a{3\a}4\a}\a5\a}{3\a}{XXX}[\cmd]|
\exemple|\detokenize\expandafter{\cmd}|
\exemple|\StrSubstitute{a1{b1\bgroup c1}\egroup d1}{1}{X}[\cmd]|
\exemple|\detokenize\expandafter{\cmd}|\smallskip

\chapitre{La macro}{StrDel}

\exemple|\noexploregroups|
\exemple|\StrDel{\a1{2\a{3\a}4\a}\a5\a}{\a}[\cmd]|
\exemple|\detokenize\expandafter{\cmd}|\vskip0.7ex
\exemple|\StrDel[2]{\a1{2\a{3\a}4\a}\a5\a}{\a}[\cmd]|
\exemple|\detokenize\expandafter{\cmd}|\vskip0.7ex
\exemple|\StrDel{\a1{2\a{3\a}4\a}\a5\a}{2}[\cmd]|
\exemple|\detokenize\expandafter{\cmd}|\vskip0.7ex
\exemple|\StrDel{\a1{2\a{3\a}4\a}\a5\a}{{3\a}}[\cmd]|
\exemple|\detokenize\expandafter{\cmd}|\vskip0.7ex
\exemple|\StrDel{\a1{2\a{3\a}4\a}\a5\a}{3\a}[\cmd]|
\exemple|\detokenize\expandafter{\cmd}|\vskip0.7ex
\exemple|\exploregroups|
\exemple|\StrDel{\a1{2\a{3\a}4\a}\a5\a}{\a}[\cmd]|
\exemple|\detokenize\expandafter{\cmd}|\vskip0.7ex
\exemple|\StrDel[2]{\a1{2\a{3\a}4\a}\a5\a}{\a}[\cmd]|
\exemple|\detokenize\expandafter{\cmd}|\vskip0.7ex
\exemple|\StrDel{\a1{2\a{3\a}4\a}\a5\a}{2}[\cmd]|
\exemple|\detokenize\expandafter{\cmd}|\vskip0.7ex
\exemple|\StrDel{\a1{2\a{3\a}4\a}\a5\a}{{3\a}}[\cmd]|
\exemple|\detokenize\expandafter{\cmd}|\vskip0.7ex
\exemple|\StrDel{\a1{2\a{3\a}4\a}\a5\a}{3\a}[\cmd]|
\exemple|\detokenize\expandafter{\cmd}|\vskip0.7ex

\chapitre{La macro}{StrLen}

\exemple|\noexploregroups|
\exemple|\StrLen{a1{a2}{\a\b}{a3}a4}|
\exemple|\exploregroups|
\exemple|\StrLen{a1{a2}{\a\b}{a3}a4}|

\chapitre{la macro}{StrSplit}

\exemple|\noexploregroups|
\exemple|\StrSplit{\a{\b{\c\d}\e}\f\g}{2}\xx\yy|
\exemple|\#\detokenize\expandafter{\xx}\#\quad\#\detokenize\expandafter{\yy}\#|
\exemple|\StrSplit{\a{\b{\c\d}\e}\f\g}{3}\xx\yy|
\exemple|\#\detokenize\expandafter{\xx}\#\quad\#\detokenize\expandafter{\yy}\#|
\exemple|\exploregroups|
\exemple|\StrSplit{\a{\b{\c\d}\e}\f\g}{2}\xx\yy|
\exemple|\#\detokenize\expandafter{\xx}\#\quad\#\detokenize\expandafter{\yy}\#|
\exemple|\StrSplit{\a{\b{\c\d}\e}\f\g}{3}\xx\yy|
\exemple|\#\detokenize\expandafter{\xx}\#\quad\#\detokenize\expandafter{\yy}\#|

\chapitre{la macro}{StrMid}

La commande {\tt\string\StrMid} opère en mode {\tt\string\noexploregroups}, quelque soit le mode d'exploration en cours.\vskip0.7ex

\exemple|\StrMid{\a\b{\c\d}\e\f\g\h}{2}{6}[\cmd]|
\exemple|\detokenize\expandafter{\cmd}|\vskip0.7ex
\exemple|\StrMid{\a\b{\c\d}\e\f\g\h}{3}{4}[\cmd]|
\exemple|\detokenize\expandafter{\cmd}|\vskip0.7ex

\chapitre{La macro}{StrGobbleLeft}

\exemple|\noexploregroups|
\exemple|\StrGobbleLeft{\a\b{\c\d\e}\f}{3}[\cmd]|
\exemple|\detokenize\expandafter{\cmd}|\vskip0.7ex
\exemple|\exploregroups|
\exemple|\StrGobbleLeft{\a\b{\c\d\e}\f}{3}[\cmd]|
\exemple|\detokenize\expandafter{\cmd}|

\chapitre{La macro}{StrGobbleRight}

\exemple|\noexploregroups|
\exemple|\StrGobbleRight{\a\b{\c\d\e}\f}{3}[\cmd]|
\exemple|\detokenize\expandafter{\cmd}|\vskip0.7ex
\exemple|\exploregroups|
\exemple|\StrGobbleRight{\a\b{\c\d\e}\f}{3}[\cmd]|
\exemple|\detokenize\expandafter{\cmd}|\vskip0.7ex

\chapitre{La macro}{StrLeft}

\exemple|\noexploregroups|
\exemple|\StrLeft{\a\b{\c\d\e}\f}{3}[\cmd]|
\exemple|\detokenize\expandafter{\cmd}|\vskip0.7ex
\exemple|\exploregroups|
\exemple|\StrLeft{\a\b{\c\d\e}\f}{3}[\cmd]|
\exemple|\detokenize\expandafter{\cmd}|

\chapitre{La macro}{StrRight}

\exemple|\noexploregroups|
\exemple|\StrRight{\a\b{\c\d\e}\f}{3}[\cmd]|
\exemple|\detokenize\expandafter{\cmd}|\vskip0.7ex
\exemple|\exploregroups|
\exemple|\StrRight{\a\b{\c\d\e}\f}{3}[\cmd]|
\exemple|\detokenize\expandafter{\cmd}|\vskip0.7ex

\chapitre{la macro}{StrChar}

\exemple|\noexploregroups|
\exemple|\StrChar{\a\b{\c\d\e}\f}{3}[\cmd]|
\exemple|\detokenize\expandafter{\cmd}|\vskip0.7ex
\exemple|\exploregroups|
\exemple|\StrChar{\a\b{\c\d\e}\f}{3}[\cmd]|
\exemple|\detokenize\expandafter{\cmd}|\vskip0.7ex

\chapitre{La macro}{StrCount}

\exemple|\noexploregroups|
\exemple|\StrCount{\a1{\a2{\a3\a4}\a5}\a6\a7}{\a}|
\exemple|\StrCount{\a1{\a2{\a3\a4}\a5}\a6\a7}{2}|
\exemple|\exploregroups|
\exemple|\StrCount{\a1{\a2{\a3\a4}\a5}\a6\a7}{\a}|
\exemple|\StrCount{\a1{\a2{\a3\a4}\a5}\a6\a7}{2}|

\chapitre{La macro}{StrPosition}

\exemple|\noexploregroups|
\exemple|\StrPosition[3]{\a0\a1{\a{2\a3}4}\a5\a6}{\a}|
\exemple|\StrPosition[4]{\a0\a1{\a{3\a4}5}\a6\a7}{\a}|
\exemple|\StrPosition[1]{\a0\a1{\a{2\a3}4}\a5\a6}{2}|
\exemple|\exploregroups|
\exemple|\StrPosition[3]{\a0\a1{\a{2\a3}4}\a5\a6}{\a}|
\exemple|\StrPosition[4]{\a0\a1{\a{2\a3}4}\a5\a6}{\a}|
\exemple|\StrPosition[1]{\a0\a1{\a{2\a3}4}\a5\a6}{2}|

\chapitre{La macro}{StrCompare}

La commande {\tt\string\StrCompare} n'est pas affectée par le mode d'exploration.\vskip0.7ex

\exemple|\comparenormal|
\exemple|\StrCompare{\a{\b1}\c2}{\a\b1\c2}|
\exemple|\StrCompare{{1\a2}3}{{1\a2}3}|
\exemple|\StrCompare{{1\a2}3}{1\a23}|
\exemple|\StrCompare{\a{\b\c}}{\a{\b\c}\d}|
\exemple|\StrCompare{{\a}\b}{\a\b}|
\exemple|\comparestrict|
\exemple|\StrCompare{\a{\b1}\c2}{\a\b1\c2}|
\exemple|\StrCompare{{1\a2}3}{{1\a2}3}|
\exemple|\StrCompare{{1\a2}3}{1\a23}|
\exemple|\StrCompare{\a{\b\c}}{\a{\b\c}\d}|
\exemple|\StrCompare{{\a}\b}{\a\b}|

\chapitre{La macro}{StrRemoveBraces}

\exemple|\noexploregroups|
\exemple|\StrRemoveBraces{\a1{\b2{\c3{\d4}}}\e5}[\cmd]|
\exemple|\detokenize\expandafter{\cmd}|\vskip0.7ex
\exemple|\exploregroups|
\exemple|\StrRemoveBraces{\a1{\b2{\c3{\d4}}}\e5}[\cmd]|
\exemple|\detokenize\expandafter{\cmd}|\vskip0.7ex
\end

==> xstring/xstring.tex <==
% !TeX encoding = ISO-8859-1
% Ce fichier contient le code de l'extension "xstring"
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                                    %
\def\xstringname               {xstring}                             %
\def\xstringversion              {1.83}                              %
%                                                                    %
\def\xstringdate              {2019/02/06}                           %
%                                                                    %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                                    %
% Author     : Christian Tellechea                                   %
% Status     : Maintained                                            %
% Maintainer : Christian Tellechea                                   %
% Email      : unbonpetit@netc.fr                                    %
% Package URL: https://www.ctan.org/pkg/xstring                      %
% Bug tracker: https://framagit.org/unbonpetit/xstring/issues        %
% Repository : https://framagit.org/unbonpetit/xstring/tree/master   %
% Copyright  : Christian Tellechea 2008-2019                         %
% Licence    : Released under the LaTeX Project Public License v1.3c %
%              or later, see http://www.latex-project.org/lppl.txt   %
% Files      : 1) xstring.tex                                        %
%              2) xstring.sty                                        %
%              3) xstring-fr.tex                                     %
%              4) xstring-fr.pdf                                     %
%              5) xstring-en.tex                                     %
%              6) xstring-en.pdf                                     %
%              7) README                                             %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\ifdefined\usepackage\else
	\immediate\write-1 {Package: xstring \xstringdate\space v\xstringversion\space String manipulations (CT)}%
\fi
\newcount\integerpart
\newcount\decimalpart% compteurs utilisés par xstring

\edef\restorexstringcatcode{\catcode\number`\_ =\number\catcode`\_\relax}
\catcode`\_=11

\long\def\xs_execfirst#1#2{#1}
\long\def\xs_execsecond#1#2{#2}
\long\def\xs_gobarg#1{}
\expandafter\def\expandafter\xs_gobspace\space{}
\def\xs_deftok#1#2{\let#1= #2\relax}\xs_deftok\xs_sptoken{ }
\long\def\xs_ifnxttok#1#2#3{\xs_deftok\xs_toksmatch{#1}\def\__truecode{#2}\def\__falsecode{#3}\xs_ifnxttok_a}
\def\xs_ifnxttok_a{\futurelet\__futurtok\xs_ifnxttok_b}
\def\xs_ifnxttok_b{%
	\xs_ifx{\__futurtok\xs_sptoken}
		{\afterassignment\xs_ifnxttok_a\let\__futurtok= }
		{\xs_ifx{\__futurtok\xs_toksmatch}\__truecode\__falsecode}%
}
\def\xs_ifstar#1{\xs_ifnxttok*{\xs_execfirst{#1}}}
\long\def\xs_testopt#1#2{\xs_ifnxttok[{#1}{#1[{#2}]}}
\long\def\xs_exparg#1#2{\expandafter\xs_exparg_a\expandafter{#2}{#1}}%
\long\def\xs_exparg_a#1#2{#2{#1}}
\long\def\xs_exptwoargs#1#2#3{\xs_exparg{\xs_exparg{#1}{#2}}{#3}}
\long\def\xs_eearg#1#2{\xs_exparg{\xs_exparg{#1}}{#2}}
\long\def\xs_edefaddtomacro#1#2{\edef#1{\unexpanded\expandafter{#1}#2}}
\long\def\xs_addtomacro#1#2{\xs_exparg{\def#1}{#1#2}}
\long\def\xs_eaddtomacro#1#2{\xs_exparg{\xs_addtomacro#1}{#2}}
\long\def\xs_eeaddtomacro#1#2{\xs_exparg{\xs_eaddtomacro#1}{#2}}
\long\def\xs_endgroup_eaddtomacro#1#2{\xs_exparg{\endgroup\xs_addtomacro#1}{#2}}
\long\def\xs_beforespace#1 #2\_nil{#1}
\long\def\xs_afterspace#1 #2\_nil{#2}
\long\def\xs_gobtonil#1\_nil{}
\long\def\xs_gobtobrace#1#{}
\long\def\xs_ifx#1{\ifx#1\expandafter\xs_execfirst\else\expandafter\xs_execsecond\fi}
\def\xs_ifnum#1{\ifnum#1\expandafter\xs_execfirst\else\expandafter\xs_execsecond\fi}
\long\def\xs_ifempty#1{\expandafter\xs_ifx\expandafter{\expandafter\relax\detokenize{#1}\relax}}

\def\xs_toks_toverb{% lit 1 argument et le transforme en verb
	\begingroup
		\def\do##1{\catcode`##112 }%
		\dospecials
		\obeyspaces
		\xs_read_verb
}

\def\setverbdelim#1{% définit quel est le délimiteur de verb
	\xs_exparg\xs_ifempty{\xs_gobarg#1}%
		{}
		{\errmessage{Package xstring Warning: verb delimiter "\detokenize{#1}" is not a single token}}%
	\def\xs_read_verb##1#1##2#1{\endgroup\xs_assign_verb{##2}}% on appelle l'exécution de fin
}

% Assigne l'argument entre délimiteur verb dans la sc #1
\def\verbtocs#1{%
	\def\xs_assign_verb##1{\def#1{##1}}%
	\xs_toks_toverb
}

\begingroup
	\catcode0 3 \gdef\xs_twozeroschars{^^00}%
	\catcode0 7 \xdef\xs_twozeroschars{\xs_twozeroschars^^00}%
\endgroup

\edef\xs_reserved_A{\long\def\noexpand\xs_assigntokenizeresult##1\xs_twozeroschars}
\xs_reserved_A#2{\endgroup\xs_exparg{\def#2}{\xs_gobarg#1}}

\def\tokenize#1#2{%
	\begingroup
		\xs_def\xs_reserved_A{#2}% on développe en accord avec \fullexpandarg ou \noexpandarg
		\everyeof\expandafter{\xs_twozeroschars#1}%
		\endlinechar-1
		\expandafter\xs_assigntokenizeresult\scantokens\expandafter{\expandafter\relax\xs_reserved_A}% on fait l'assignation
}%

\long\def\xs_assign_xstringresult#1#2{\xs_ifempty{#2}{#1}{\def#2{#1}}}

\def\xs_ldef{\long\def}
\def\xs_ledef{\long\edef}

\def\normalexpandarg{%
	\let\xs_def\xs_ldef% on définit \xs_call avec \def
	\def\xs_expand##1{\unexpanded\expandafter{##1}}%
}
\let\noexpandarg\normalexpandarg% synonyme

\def\expandarg{%
	\let\xs_def\xs_ldef% on définit \xs_call avec \def
	\def\xs_expand##1{\unexpanded\expandafter\expandafter\expandafter{##1}}%
}

\def\fullexpandarg{%
	\let\xs_def\xs_ledef% on définit\xs_call avec \edef
	\def\xs_expand##1{##1}% et on neutralise \xs_expand
}

\def\saveexpandmode{\let\xs_saved_def\xs_defarg\let\xs_saved_expand\xs_expand}
\def\restoreexpandmode{\let\xs_defarg\xs_saved_def\let\xs_expand\xs_saved_expand}

% Macro interne renvoyant #2 si son argument commence par une accolade ouvrante "{"
% et #3 sinon (Ulrich Diez sur comp.text.tex)
\long\def\xs_ifbeginwithbrace#1{%
	\csname xs_exec%
		\expandafter\xs_gobarg\string{%
		\expandafter\xs_gobarg\expandafter{\expandafter{\string#1}%
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\xs_execfirst
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\xs_gobarg
		\expandafter\expandafter\expandafter\xs_gobarg
		\expandafter\expandafter\expandafter{\expandafter\string\expandafter}\string}%
		\expandafter\xs_gobarg\string}%
		\xs_execsecond{first}{second}%
	\endcsname
}

% Cette macro interne prend la 1ere unité syntaxique de #1 et assigne le résultat à #2
\long\def\xs_returnfirstsyntaxunit#1#2{%
	\let\xs_toks\relax
	\xs_ifempty{#1}
		{\let#2\empty
		}
		{\xs_eearg\xs_ifempty{\expandafter\xs_beforespace\detokenize{#1} \_nil}% #1 commence par un espace ?
			{\def#2{ }}
			{\xs_ifbeginwithbrace{#1}
				{\def\xs_groupfound{\xs_exparg{\def#2}{\expandafter{#2}}\xs_gobtonil}% on met #2 dans des accolades et on finit
				\let\xs_toks\bgroup
				\afterassignment\xs_groupfound
				\def#2%
				}
				{\long\def\xs_assignfirstarg##1##2\_nil{\def#2{##1}}%
				\xs_assignfirstarg
				}%
			#1\_nil
			}%
		}%
}

\long\def\xs_removefirstsyntaxunit#1#2{%
	\xs_ifempty{#1}
		{\let#2\empty
		}
		{\xs_eearg\xs_ifempty{\expandafter\xs_beforespace\detokenize{#1} \_nil}% #1 commence par un espace ?
			{\xs_exparg\xs_ifbeginwithbrace{\xs_gobspace#1}
				{\xs_exparg{\def#2}{\xs_gobtobrace#1}}%
				{\xs_exparg{\def#2}{\xs_afterspace#1\_nil}}%
			}%
			{\xs_exparg{\def#2}{\xs_gobarg#1}}%
		}%
}

% Cette macro interne est utilisée dans les macros étoilées pour :
% 1) développer l'argument selon qu'on a choisit \fullexpandarg
%    ou \normalexpandarg, et ceci à l'aide de la macro \xs_def
% 2) Ensuite, on détokenize ce développement de façon n'avoir plus que
%    des catcodes de 10 pour les espaces et 12 pour le reste.
\long\def\xs_expand_and_detokenize#1#2{%
	\long\def#1{#2}%
	\expandafter\edef\expandafter#1\expandafter{\xs_expand#1}% on développe #2 selon le mode de développement
	\long\edef#1{\detokenize\expandafter{#1}}% puis on détokenize et on assigne à #1
}

\long\def\xs_expand_and_assign#1#2{\xs_def#1{#2}}% on développe #2 selon \fullexpandarg ou \normalexpandarg

\def\xs_arglist{0########1########2########3########4########5########6########7########8########9}

% \xs_assign_args{3} met dans la sc \xs_myarg les tokens "####1####2####3"
\def\xs_assign_args#1{\def\xs_assign_args_i0##1#1##2\_nil{\def\xs_myarg{##1#1}}\expandafter\xs_assign_args_i\xs_arglist\_nil}

% \xs_assign_opt_args{3} met dans la sc \xs_myarg les tokens "[####1]####2####3####4"
\def\xs_assign_opt_args#1{\xs_exparg\xs_assign_opt_args_i{\number\numexpr#1+1}}
\def\xs_assign_opt_args_i#1{\def\xs_assign_opt_args_ii0##11##2#1##3\_nil{\def\xs_myarg{[##11]##2#1}}\expandafter\xs_assign_opt_args_ii\xs_arglist\_nil}

% \xs_assign_one_arg{3} met dans la sc \xs_myarg les tokens "####3"
\def\xs_assign_one_arg#1{\xs_exparg\xs_assign_one_arg_i{\number\numexpr#1-1}{#1}}
\def\xs_assign_one_arg_i#1#2{\def\xs_assign_one_arg_ii##1#1##2#2##3\_nil{\def\xs_myarg{##2#2}}\expandafter\xs_assign_one_arg_ii\xs_arglist\_nil}

% #1 : numéro du 1er argument; #2 : nombre de lignes; #3 argument optionnel; #4 : dernier numéro de l'argument devant être détokenisé si étoile
\def\xs_buildlines#1#2#3#4{%
	\let\xs_newlines\empty
	\let\xs_newargs\empty
	\def\xs_buildlines_i##1{%
		\xs_exparg\xs_assign_one_arg{\number\numexpr##1+#1-1}%
		\edef\xs_reserved_B{\noexpand\xs_expand\csname xs_arg_\romannumeral\numexpr##1\endcsname}%
		\xs_ifnum{##1=1 }% si c'est le premier argument
			{\xs_ifempty{#3}%
				{\xs_eaddtomacro\xs_newargs{\expandafter{\xs_reserved_B}}%
				\edef\xs_reserved_B{\ifnum##1>#4 xs_def\else xs_assign\fi}%
				}% et s'il y a un argument optionnel alors, on met des crochets
				{\xs_eaddtomacro\xs_newargs{\expandafter[\xs_reserved_B]}%
				\def\xs_reserved_B{xs_def}% ne pas détokéniser l'argument optionnel grace au \xs_def
				}%
			}
			{\xs_eaddtomacro\xs_newargs{\expandafter{\xs_reserved_B}}%
			\edef\xs_reserved_B{\ifnum##1>#4 xs_def\else xs_assign\fi}%
			}%
		\edef\xs_newlines{\unexpanded\expandafter{\xs_newlines}\expandafter\noexpand\csname\xs_reserved_B\endcsname\expandafter\noexpand\csname xs_arg_\romannumeral\numexpr##1\endcsname{\xs_myarg}}%
		\xs_ifnum{##1<#2 }
			{\xs_exparg\xs_buildlines_i{\number\numexpr##1+1}}
			{}%
	}%
	\xs_buildlines_i1%
}

\def\xs_newmacro{%
	\xs_ifstar
		{\let\xs_reserved_D\empty\xs_newmacro_}
		{\let\xs_reserved_D\relax\xs_newmacro_0}%
}

% #1 : dernier numéro de l'argument devant être détokenisé
% #2 : nom de la macro publique
% #3 : argument optionnel (vide si pas d'arg optionnel)
% #4 : nombre d'arguments obligatoires
% #5 : utilisation de testopt (1 si oui, 0 si non)
% #6 : code de la macro
\def\xs_newmacro_#1#2#3#4#5{%
	\edef\xs_reserved_A{xs_\expandafter\xs_gobarg\string#2}%
	\edef\xs_reserved_C{\expandafter\noexpand\csname\xs_reserved_A _\ifx\empty#3\empty _\fi\endcsname}%
	\edef\xs_reserved_B{%
		\long
		\ifx\empty\xs_reserved_D
			\def\noexpand#2{\noexpand\xs_ifstar
				{\let\noexpand\xs_assign\noexpand\xs_expand_and_detokenize\expandafter\noexpand\xs_reserved_C}%
				{\let\noexpand\xs_assign\noexpand\xs_expand_and_assign\expandafter\noexpand\xs_reserved_C}%
			}%
		\else
			\def\noexpand#2{\let\noexpand\xs_assign\noexpand\xs_expand_and_assign\expandafter\noexpand\xs_reserved_C}%
		\fi
		\ifx\empty#3\empty
		\else
			\def\expandafter\noexpand\xs_reserved_C{%
				\noexpand\xs_testopt{\expandafter\noexpand\csname\xs_reserved_A __\endcsname}{\ifx\xs_def\xs_ledef#3\else\unexpanded{#3}\fi}}%
		\fi
	}%
	% Que fait \xs_reserved_B ? Il définit :
	% si #3 est vide : \NOM{\xs_ifstar{\let\xs_assign\xs_expand_and_detokenize\xs_NOM__}{\let\xs_assign\xs_expand_and_assign\xs_NOM__}}
	% si #3 existe   : \NOM{\xs_ifstar{\let\xs_assign\xs_expand_and_detokenize\xs_NOM_}{\let\xs_assign\xs_expand_and_assign\xs_NOM_}}
	%                  \xs_NOM_{\xs_testopt{\xs_NOM__}{#3}}}
	\xs_reserved_B
	\ifx\empty#3\empty
		\xs_buildlines1{#4}{#3}{#1}%
		\xs_assign_args{#4}%
	\else
		\xs_exparg{\xs_buildlines1}{\number\numexpr#4+1}{#3}{#1}%
		\xs_assign_opt_args{#4}%
	\fi
	\edef\xs_reserved_B{\def\expandafter\noexpand\csname\xs_reserved_A __\endcsname\xs_myarg}%
	\edef\xs_reserved_C{\unexpanded\expandafter{\xs_newlines}\edef\noexpand\xs_call}%
	\edef\xs_reserved_D{\noexpand\noexpand\expandafter\noexpand\csname\xs_reserved_A\endcsname\unexpanded\expandafter{\xs_newargs}}%
	\ifnum#5=1 \edef\xs_reserved_D{\noexpand\noexpand\noexpand\xs_testopt{\unexpanded\expandafter{\xs_reserved_D}}{}}\fi
	\xs_edefaddtomacro\xs_reserved_C{{\unexpanded\expandafter{\xs_reserved_D}}\noexpand\xs_call}%
	\xs_edefaddtomacro\xs_reserved_B{{\unexpanded\expandafter{\xs_reserved_C}}}%
	% Que fait \xs_reserved_B ? Il définit par exemple pour 3 arguments obligatoires et 1 facultatif :
	%    \def\xs_NOM__[##2]##3##4##5{%
	%          \xs_def\xs_arg_i{##2}\xs_assign\xs_arg_ii{##3}\xs_assign\xs_arg_iii{##4}\xs_asign\xs_arg_iv{##5}%
	% si #5=0: \edef\xs_call{\noexpand\xs_NOM[\xs_expand\xs_arg_i]{\xs_expand\xs_arg_ii}{\xs_expand\xs_arg_iii}{\xs_expand\xs_arg_iv}}%
	% si #5=1: \edef\xs_call{\noexpand\xs_testopt{\noexpand\xs_NOM[\xs_expand\xs_arg_i]{\xs_expand\xs_arg_i}{\xs_expand\xs_arg_ii}{\xs_expand\xs_arg_iii}{\xs_expand\xs_arg_iv}}{}}%
	%          \xs_call}
	\long\xs_reserved_B
	\edef\xs_reserved_B{%
		\def\expandafter\noexpand\csname\xs_reserved_A\endcsname
			\xs_myarg\ifnum#5=1 [\unexpanded{##}\number\numexpr\ifx\empty#3\empty#4+1\else#4+2\fi]\fi
	}%
	% Que fait \xs_reserved_B ? Il définit par exemple pour 3 arguments obligatoires et 1 facultatif :
	%    \def \xs_NOM[##2]##3##4##5[##6]{#6}
	\long\xs_reserved_B
}

% macro générique qui lit \xs_reserved_C us par us
% 3 sous-routines sont appelées à des moments clé :
% \xs_atendofgroup      (un groupe se finit, appel récursif)
% \xs_atbegingroup      (un groupe vient d'être ouvert)
% \xs_atnextsyntaxunit  (la future US n'est pas un groupe)
\def\xs_read_reserved_C{%
	\xs_exparg\xs_ifempty{\xs_reserved_C}%
		{\xs_ifnum{\xs_nestlevel=0 }
			{}
			{\xs_atendofgroup
			\xs_read_reserved_C
			}%
		}
		{\xs_exparg\xs_returnfirstsyntaxunit{\xs_reserved_C}\xs_reserved_A
		\xs_exparg\xs_removefirstsyntaxunit{\xs_reserved_C}\xs_reserved_C
		\xs_exploregroups
		\xs_ifx{\bgroup\xs_toks}
			{\advance\integerpart1
			\begingroup
				\expandafter\def\expandafter\xs_reserved_C\xs_reserved_A
				\xs_calc_grouIP
				\def\xs_nestlevel{1}%
				\integerpart0
				\xs_atbegingroup
			}
			{\advance\decimalpart1
			\xs_atnextsyntaxunit
			}%
		\xs_read_reserved_C
		}%
}

% macro générique qui lit \xs_reserved_D en procédant à des tests avec \IfBeginWith
% 1 sous-routine est appelée :
% \xs_atoccurfound      (une occurrence a été trouvée)
\def\xs_read_reserved_D{%
	\xs_exparg\xs_ifempty{\xs_reserved_D}%
		{\xs_ifnum{\xs_nestlevel=0 }
			{}
			{\edef\__temp{%
				\endgroup
				\noexpand\decimalpart=\number\decimalpart\relax
				\unexpanded{\xs_addtomacro\xs_reserved_C}{{\unexpanded\expandafter{\xs_reserved_C}}}%
				}%
			\__temp
			\xs_read_reserved_D
			}%
		}%
		{\xs_exptwoargs\xs_IfBeginWith_i\xs_reserved_D\xs_reserved_E
			{\advance\decimalpart1
			\let\xs_reserved_D\xs_reserved_A
			\xs_atoccurfound
			}%
			{\xs_exparg\xs_returnfirstsyntaxunit{\xs_reserved_D}\xs_reserved_A
			\xs_exparg\xs_removefirstsyntaxunit{\xs_reserved_D}\xs_reserved_D
			\xs_exploregroups
			\xs_ifx{\bgroup\xs_toks}
				{\advance\integerpart1
				\begingroup
					\expandafter\def\expandafter\xs_reserved_D\xs_reserved_A
					\xs_calc_grouIP
					\let\xs_reserved_C\empty
					\def\xs_nestlevel{1}%
					\integerpart0
				}
				{\xs_eaddtomacro\xs_reserved_C{\xs_reserved_A}%
				}%
			}%
		\xs_read_reserved_D
		}%
}

\xs_newmacro\StrRemoveBraces{}{1}{1}{%
	\def\xs_reserved_C{#1}%
	\let\xs_reserved_B\empty
	\def\xs_nestlevel{0}%
	\xs_StrRemoveBraces_i
	\xs_exparg\xs_assign_xstringresult{\xs_reserved_B}{#2}%
}

\def\xs_StrRemoveBraces_i{%
	\xs_exparg\xs_ifempty{\xs_reserved_C}%
		{\xs_ifnum{\xs_nestlevel=0 }
			{}
			{\xs_endgroup_eaddtomacro\xs_reserved_B\xs_reserved_B
			\xs_StrRemoveBraces_i
			}%
		}
		{\xs_exparg\xs_returnfirstsyntaxunit{\xs_reserved_C}\xs_reserved_A
		\xs_exparg\xs_removefirstsyntaxunit{\xs_reserved_C}\xs_reserved_C
		\xs_ifx{\bgroup\xs_toks}
			{\xs_ifx{\xs_exploregroups\relax}% on explore les groupes ?
				{\begingroup
					\expandafter\def\expandafter\xs_reserved_C\xs_reserved_A
					\def\xs_nestlevel{1}%
					\let\xs_reserved_B\empty
				}
				{\expandafter\xs_addtomacro\expandafter\xs_reserved_B\xs_reserved_A
				}%
			}
			{\xs_eaddtomacro\xs_reserved_B{\xs_reserved_A}%
			}%
		\xs_StrRemoveBraces_i
		}%
}

% \xs_cutafteroccur coupe l'argument #1 après la #3ème occurrence de #2
% \xs_reserved_C : contient ce qui se trouve avant cette occurrence
% \xs_reserved_D : contient ce qui se trouve avant cette occurrence y compris cette occurrence
% \xs_reserved_E : contient ce qui se trouve après l'occurrence
% si l'occurrence n'existe pas ou qu'un des arguments est vide, toutes les chaines renvoyées sont vides
\long\def\xs_cutafteroccur#1#2#3{%
	\xs_ifnum{#3<1 }
		{\let\xs_reserved_C\empty\let\xs_reserved_E\empty\gdef\groupID{}}
		{\xs_cutafteroccur_i{#1}{#2}{#3}}%
}
	
\long\def\xs_cutafteroccur_i#1#2#3{%
	\def\xs_reserved_D{#1}\let\xs_reserved_C\empty\def\xs_reserved_E{#2}%
	\decimalpart0 \integerpart0 \gdef\groupID{0}\def\xs_nestlevel{0}%
	\def\xs_atoccurfound{%
		\xs_ifnum{\decimalpart=\numexpr(#3)\relax}
			{\edef\__temp{%
				\def\noexpand\xs_reserved_C{\unexpanded\expandafter{\xs_reserved_C}}%
				\def\noexpand\xs_reserved_D{\unexpanded\expandafter{\xs_reserved_D}}%
				\noexpand\decimalpart=\number\decimalpart\relax
				}%
			\expandafter\xs_exitallgroups\__temp
			\xs_gobarg% mange l'appel récursif \xs_read_reserved_D dans \xs_read_reserved_D
			}
			{\xs_eaddtomacro\xs_reserved_C{\xs_reserved_E}%
			}%
	}%
	\xs_read_reserved_D
	\xs_ifnum{\decimalpart=\numexpr(#3)\relax}% occurrence trouvée ?
		{\let\xs_reserved_E\xs_reserved_D
		\xs_exparg{\def\xs_reserved_D}{\xs_reserved_C#2}%
		}
		{\let\xs_reserved_C\empty
		\let\xs_reserved_E\empty
		\gdef\groupID{}%
		}%
}

\xs_newmacro*3\IfSubStr{1}{2}{0}{%
	\xs_cutafteroccur{#2}{#3}{#1}%
	\xs_exparg\xs_ifempty{\xs_reserved_D}\xs_execsecond\xs_execfirst
}

\xs_newmacro*2\IfBeginWith{}{2}{0}{%
	\xs_ifempty{#2}%
		{\xs_execsecond}
		{\xs_IfBeginWith_i{#1}{#2}}%
}

\long\def\xs_IfBeginWith_i#1#2{%
	\xs_ifempty{#2}%
		{\xs_execfirst% #2 est vide, tous les tests sont passés avec succès : on renvoie #3
		}
		{\xs_ifempty{#1}%
			{\xs_execsecond% #1 est vide, c'est que #2 est + long que #1 : on renvoie #4
			}
			{\xs_returnfirstsyntaxunit{#2}\xs_reserved_B
			\xs_returnfirstsyntaxunit{#1}\xs_reserved_A
			\xs_ifx{\xs_reserved_A\xs_reserved_B}% il y a égalité...
				{\xs_removefirstsyntaxunit{#2}\xs_reserved_B
				\xs_removefirstsyntaxunit{#1}\xs_reserved_A% on enlève les 1ere unités syntaxiques
				\xs_exptwoargs\xs_IfBeginWith_i\xs_reserved_A\xs_reserved_B
				}
				{\xs_execsecond
				}%
			}%
		}%
}

\xs_newmacro*2\IfEndWith{}{2}{0}{%
	\xs_ifempty{#2}%
		{\xs_execsecond
		}
		{\xs_StrCount{#1}{#2}[\xs_reserved_A]%
		\xs_ifnum{\xs_reserved_A=0 }
			{\xs_execsecond}
			{\xs_exparg\xs_ifempty{\xs_reserved_C}}%
		}%
}

\xs_newmacro*4\IfSubStrBefore{1,1}{3}{0}{\xs_IfSubStrBefore_i[#1]{#2}{#3}{#4}}

\def\xs_IfSubStrBefore_i[#1,#2]#3#4#5{%
	\def\xs_reserved_C{#3}%
	\xs_ifx{\xs_exploregroups\relax}% si on explore les groupes
		{\let\xs_reserved_B\empty
		\def\xs_nestlevel{0}%
		\xs_StrRemoveBraces_i% on retire les accolades
		\let\xs_reserved_C\xs_reserved_B
		}
		{}%
	\xs_exparg\xs_cutafteroccur\xs_reserved_C{#5}{#2}%
	\xs_exparg\xs_cutafteroccur\xs_reserved_C{#4}{#1}%
	\gdef\groupID{}%
	\xs_exparg\xs_ifempty{\xs_reserved_C}%
		\xs_execsecond
		\xs_execfirst
}

\xs_newmacro*4\IfSubStrBehind{1,1}{3}{0}{\xs_IfSubStrBehind_i[#1]{#2}{#3}{#4}}
\long\def\xs_IfSubStrBehind_i[#1,#2]#3#4#5{\xs_IfSubStrBefore_i[#2,#1]{#3}{#5}{#4}}

\long\def\xs_formatnumber#1#2{%
	\xs_ifempty{#1}%
		{\def#2{0X}% si vide, renvoie 0X
		}
		{\xs_returnfirstsyntaxunit{#1}\xs_reserved_A
		\def\xs_reserved_B{+}%
		\xs_ifx{\xs_reserved_A\xs_reserved_B}
			{\xs_removefirstsyntaxunit{#1}\xs_reserved_C
			\xs_exparg\xs_ifempty{\xs_reserved_C}%
				{\def#2{+0X}}
				{\xs_exparg{\def#2}{\expandafter+\expandafter0\xs_reserved_C}}%
			}
			{\def\xs_reserved_B{-}%
			\xs_ifx{\xs_reserved_A\xs_reserved_B}
				{\xs_removefirstsyntaxunit{#1}\xs_reserved_A
				\xs_exparg\xs_ifempty{\xs_reserved_A}%
					{\def#2{-0X}}%
					{\xs_exparg{\def#2}{\expandafter-\expandafter0\xs_reserved_A}}%
				}
				{\def#2{0#1}%
				}%
			}%
		}%
}

\xs_newmacro\IfInteger{}{1}{0}{%
	\xs_formatnumber{#1}\xs_reserved_A
	\decimalpart0
	\afterassignment\xs_defafterinteger\integerpart\xs_reserved_A\relax\_nil
	\let\xs_after_intpart\afterinteger
	\expandafter\xs_testdot\afterinteger\_nil
	\xs_ifx{\empty\afterdecimal}
		{\xs_ifnum{\decimalpart=0 }
			{\xs_execfirst% partie décimale constituée de 0 --> seul cas où on renvoie vrai
			}
			{\expandafter\xs_defafterinteger\xs_after_intpart\relax\_nil
			\xs_execsecond
			}%
		}
		{\expandafter\xs_defafterinteger\xs_after_intpart\relax\_nil
		\xs_execsecond
		}%
}

\xs_newmacro\IfDecimal{}{1}{0}{%
	\xs_formatnumber{#1}\xs_reserved_A
	\decimalpart0
	\afterassignment\xs_defafterinteger\integerpart\xs_reserved_A\relax\_nil
	\expandafter\xs_testdot\afterinteger\_nil
	\xs_ifx{\empty\afterdecimal}
}

\begingroup\catcode`\@ 11
\long\gdef\xs_defafterinteger#1\relax\_nil{\def\@xs@afterinteger{#1}\let\afterinteger\@xs@afterinteger}
\long\gdef\xs_defafterdecimal#1\_nil{\def\@xs@afterdecimal{#1}\let\afterdecimal\@xs@afterinteger}
\endgroup

\def\xs_testdot{%
	\let\xs_decsep\empty
	\xs_ifnxttok.
		{\def\xs_decsep{.}\xs_readdecimalpart}%
		{\xs_testcomma}%
}

\def\xs_testcomma{%
	\xs_ifnxttok,
		{\def\xs_dessep{,}\xs_readdecimalpart}%
		{\xs_defafterdecimal}%
}

\long\def\xs_readdecimalpart#1#2\_nil{%
	\xs_ifempty{#2}
		{\def\xs_reserved_A{0X}}
		{\def\xs_reserved_A{0#2}}%
	\afterassignment\xs_defafterinteger\decimalpart\xs_reserved_A\relax\_nil
	\expandafter\xs_defafterdecimal\afterinteger\_nil
}

% test d'égalité sur des chaines (et des chaines contenant des nombres)
\long\def\xs_IfStrEqFalse_i#1#2{\let\xs_reserved_A\xs_execsecond}
\long\def\xs_IfStrEqFalse_ii#1#2{% renvoie vrai si les 2 arg sont décimaux et s'ils sont égaux, faux sinon
	\xs_IfDecimal{#1}%
		{\xs_IfDecimal{#2}%
			{\ifdim#1pt=#2pt
				\let\xs_reserved_A\xs_execfirst
			\else
				\let\xs_reserved_A\xs_execsecond
			\fi% les 2 sont décimaux : on fait le test
			}%
			{\let\xs_reserved_A\xs_execsecond}% un seul est décimal
		}%
		{\let\xs_reserved_A\xs_execsecond}% #1 n'est pas décimal
}

\long\def\xs_TestEqual#1#2{% teste si les 2 arguments sont égaux
	\def\xs_reserved_A{#1}\def\xs_reserved_B{#2}%
	\xs_ifx{\xs_reserved_A\xs_reserved_B}
		{\let\xs_reserved_A\xs_execfirst}% égalité parfaite des 2 chaines
		{\xs_reserved_D{#1}{#2}}%
	\xs_reserved_A
}

\xs_newmacro*2\IfStrEq{}{2}{0}{% teste si les deux chaines sont égales
	\let\xs_reserved_D\xs_IfStrEqFalse_i
	\xs_TestEqual{#1}{#2}%
}

\xs_newmacro*2\IfEq{}{2}{0}{% teste si les 2 arguments (chaine ou nombre) sont égaux
	\let\xs_reserved_D\xs_IfStrEqFalse_ii
	\xs_TestEqual{#1}{#2}%
}

\def\IfStrEqCase{%
	\xs_ifstar
		{\xs_IfStringCase{\IfStrEq*}}%
		{\xs_IfStringCase\IfStrEq}%
}

\def\IfEqCase{%
	\xs_ifstar
		{\xs_IfStringCase{\IfEq*}}%
		{\xs_IfStringCase\IfEq}%
}

\long\def\xs_IfStringCase#1#2#3{% #1=macro avec ou sans étoile  #2=argument à tester  #3=liste des {<cas>}{code>}
	\long\def\xs_testcase##1##2##3\_nil{% lit les 2 premieres unités syntaxiques dans ##1 et ##2. Les autres dans ##3
		#1{#2}{##1}% compare
			{\xs_testopt{\xs_IfStringCase_ii{##2}}{}}% le test est positif, on exécute le code correspondant et on mange l'argument optionnel ## BUGfix dans 1.82
			{\xs_ifempty{##3}%
				{\xs_testopt{\xs_IfStringCase_i}{}}% s'il n'y a plus de cas, on exécute le code <autres cas> ## BUGfix dans 1.82
				{\xs_testcase##3\_nil}% sinon, on recommence avec ce qui reste
			}%
	}%
	\xs_testcase#3\_nil
}

\long\def\xs_IfStringCase_i[#1]{#1}
\long\def\xs_IfStringCase_ii#1[#2]{#1}

% Renvoie ce qui est à gauche de l'occurence n°#1 de la sous chaine #3 dans la chaine #2
\xs_newmacro*3\StrBefore{1}{2}{1}{%
	\xs_cutafteroccur{#2}{#3}{#1}%
	\xs_exparg\xs_assign_xstringresult{\xs_reserved_C}{#4}%
}

% Renvoie ce qui est à droite de l'occurence n°#1 de la sous chaine #3 dans la chaine #2
\xs_newmacro*3\StrBehind{1}{2}{1}{%
	\xs_cutafteroccur{#2}{#3}{#1}%
	\xs_exparg\xs_assign_xstringresult{\xs_reserved_E}{#4}%
}

% Renvoie ce qui est strictement compris entre les occurrences n°#1 et n°#2
% des chaines #4 et #5 dans la chaine #3
\xs_newmacro*4\StrBetween{1,1}{3}{1}{\xs_StrBetween_i[#1]{#2}{#3}{#4}[#5]}
\long\def\xs_StrBetween_i[#1,#2]#3#4#5[#6]{%
	\begingroup
		\noexploregroups
		\xs_cutafteroccur{#3}{#5}{#2}%
		\xs_exparg\xs_cutafteroccur{\xs_reserved_C}{#4}{#1}%
		\expandafter
	\endgroup
	\expandafter\xs_assign_xstringresult\expandafter{\xs_reserved_E}{#6}%
	\gdef\groupID{}%
}

\def\exploregroups{\let\xs_exploregroups\relax}
\def\noexploregroups{\def\xs_exploregroups{\let\xs_toks\relax}}
\def\saveexploremode{\let\xs_saveexploremode\xs_exploregroups}
\def\restoreexploremode{\let\xs_exploregroups\xs_saveexploremode}

% Remplace les #1 premières occurences de la chaine #3
% par la chaine #4 dans la chaine #2
\xs_newmacro\StrSubstitute{0}{3}{1}{%
	\def\xs_reserved_D{#2}\let\xs_reserved_C\empty\def\xs_reserved_E{#3}%
	\decimalpart0 \integerpart0 \gdef\groupID{0}\def\xs_nestlevel{0}%
	\def\xs_atoccurfound{%
		\xs_ifnum{#1<1 }
			{\def\xs_reserved_A{#4}}
			{\xs_ifnum{\decimalpart>#1 }
				{\def\xs_reserved_A{#3}}
				{\def\xs_reserved_A{#4}}%
			}%
		\xs_eaddtomacro\xs_reserved_C{\xs_reserved_A}%
	}%
	\xs_ifempty{#3}%
		{\xs_exparg\xs_assign_xstringresult{\xs_reserved_D}{#5}%
		}
		{\xs_read_reserved_D
		\xs_exparg\xs_assign_xstringresult{\xs_reserved_C}{#5}%
		}%
}

% Supprime les #1 premières occurrences de #3 dans #2
\xs_newmacro\StrDel{0}{2}{1}{\xs_StrSubstitute[#1]{#2}{#3}{}[#4]}

\def\xs_exitallgroups{\ifnum\xs_nestlevel>0 \endgroup\expandafter\xs_exitallgroups\fi}

% Compte combien d'unités syntaxiques contient la chaine #1 ?
\xs_newmacro\StrLen{}{1}{1}{%
	\def\xs_reserved_C{#1}\decimalpart0 \def\xs_nestlevel{0}\gdef\groupID{0}%
	\let\xs_atbegingroup\relax
	\def\xs_atendofgroup{\expandafter\endgroup\expandafter\decimalpart\number\decimalpart\relax}%
	\let\xs_atnextsyntaxunit\relax
	\xs_read_reserved_C
	\xs_exparg\xs_assign_xstringresult{\number\decimalpart}{#2}%
}

% Macro interne fermant autant de groupes que nécessaire pour trouver une unité syntaxique derrière
\def\xs_continuetonext{%
	\xs_exparg\xs_ifempty{\xs_reserved_C}%
		{\ifnum\xs_nestlevel>0
			\xs_endgroup_eaddtomacro\xs_reserved_B{\expandafter{\xs_reserved_B}}% on concatène
			\expandafter\xs_continuetonext% on recommence
		\fi}
		{}%
}%

\def\xs_calc_grouIP{%
	\begingroup\def\xs_reserved_A{0}%
	\xs_ifx{\xs_reserved_A\groupID}% si on arrive du groupe de niveau 0
		{\endgroup\xdef\groupID{\number\integerpart}}% on met simplement le niveau
		{\endgroup\xs_eearg{\gdef\groupID}{\expandafter\groupID\expandafter,\number\integerpart}}%
}

% Cette macro coupe la chaine #1 après l'unité syntaxique n°#2
\def\StrSplit{%
	\xs_ifstar
		{\let\xs_reserved_E\xs_continuetonext\StrSplit_i}%
		{\let\xs_reserved_E\relax\StrSplit_i}%
}

\xs_newmacro\StrSplit_i{}{2}{0}{\xs_StrSplit_ii{#2}{#1}\xs_StrSplit_iii}

% Cette macro interne coupe la chaine #2 après l'unité syntaxique n°#1
% Le début est assigné dans \xs_reserved_B et la fin dans \xs_reserved_C
\long\def\xs_StrSplit_ii#1#2{%
	\let\xs_reserved_B\empty\def\xs_reserved_C{#2}\def\xs_reserved_D{#1}\gdef\groupID{}%
	\ifnum#1>0
		\decimalpart0 \integerpart0 \gdef\groupID{0}\def\xs_nestlevel{0}%
		\def\xs_atendofgroup{%
			\edef\__temp{%
				\endgroup
				\noexpand\decimalpart=\number\decimalpart\relax
				\unexpanded{\xs_addtomacro\xs_reserved_B}{{\unexpanded\expandafter{\xs_reserved_B}}}%
				}%
			\__temp
		}%
		\def\xs_atbegingroup{\let\xs_reserved_B\empty}%
		\def\xs_atnextsyntaxunit{%
			\xs_eaddtomacro\xs_reserved_B{\xs_reserved_A}%
			\xs_ifnum{\decimalpart=\xs_reserved_D\relax}
				{\ifx\xs_reserved_C\empty\xs_reserved_E\fi
				\edef\__temp{\def\noexpand\xs_reserved_B{\unexpanded\expandafter{\xs_reserved_B}}\def\noexpand\xs_reserved_C{\unexpanded\expandafter{\xs_reserved_C}}}%
				\expandafter\xs_exitallgroups\__temp
				\xs_gobarg% mange l'appel récursif \xs_read_reserved_C dans \xs_read_reserved_C
				}
				{}%
		}%
		\xs_read_reserved_C
	\fi
}

\def\xs_StrSplit_iii#1#2{\let#1\xs_reserved_B\let#2\xs_reserved_C}

% StrCut[n]{<texte>}{<motif>}\macroA\macroB
% \macroA reçoit ce qui se trouve avant la n ème occurrence <motif> dans <texte>
% \macroB reçoit ce qui est après cette n ème occurrence
\xs_newmacro*3\StrCut{1}{2}{0}{%
	\xs_ifempty{#3}%
		{\gdef\groupID{}\let\xs_reserved_C\empty\let\xs_reserved_E\empty
		}
		{\xs_ifnum{#1<1 }
			{\xs_StrCut_ii{#2}{#3}1}
			{\xs_StrCut_ii{#2}{#3}{#1}}%
		}%
	\xs_StrCut_iii
}

\long\def\xs_StrCut_ii#1#2#3{%
	\let\xs_reserved_C\empty\def\xs_reserved_D{#1}\def\xs_reserved_E{#2}%
	\decimalpart0 \integerpart0 \gdef\groupID{0}\def\xs_nestlevel{0}%
	\def\xs_atoccurfound{%
		\xs_ifnum{\decimalpart=\numexpr(#3)\relax}
			{\edef\__temp{%
				\def\noexpand\xs_reserved_C{\unexpanded\expandafter{\xs_reserved_C}}%
				\def\noexpand\xs_reserved_D{\unexpanded\expandafter{\xs_reserved_D}}%
				\noexpand\decimalpart=\number\decimalpart\relax
				}%
			\expandafter\xs_exitallgroups\__temp
			\xs_gobarg% stoppe la récursivité dans \xs_read_reserved_D
			}
			{\xs_eaddtomacro\xs_reserved_C{\xs_reserved_E}%
			}%
	}%
	\xs_read_reserved_D
	\let\xs_reserved_E\xs_reserved_D
	\xs_exparg{\def\xs_reserved_D}{\xs_reserved_C#2}%
}

\long\def\xs_StrCut_iii#1#2{\let#1\xs_reserved_C\let#2\xs_reserved_E}

% De la chaine #1, renvoie ce qui se trouve entre les positions
%  #2 et #3, unités syntaxiques aux positions compris !
\xs_newmacro\StrMid{}{3}{1}{%
	\begingroup
		\noexploregroups
		\let\xs_reserved_E\relax
		\xs_StrSplit_ii{#3}{#1}%
		\edef\xs_reserved_C{\number\numexpr#2-1}%
		\let\xs_reserved_E\relax
		\xs_exptwoargs\xs_StrSplit_ii\xs_reserved_C\xs_reserved_B
	\expandafter\endgroup
	\expandafter\xs_assign_xstringresult\expandafter{\xs_reserved_C}{#4}%
	\gdef\groupID{}%
}

% supprime #2 unités syntaxiques à gauche dans la chaine #1
\xs_newmacro\StrGobbleLeft{}{2}{1}{%
	\let\xs_reserved_E\relax
	\xs_StrSplit_ii{#2}{#1}%
	\xs_exparg\xs_assign_xstringresult{\xs_reserved_C}{#3}%
}

% extrait de #1 la chaine à gauche de longueur #2
\xs_newmacro\StrLeft{}{2}{1}{%
	\let\xs_reserved_E\relax
	\xs_StrSplit_ii{#2}{#1}%
	\xs_exparg\xs_assign_xstringresult{\xs_reserved_B}{#3}%
}

% supprime #2 unités syntaxiques à droite dans la chaine #1
\xs_newmacro\StrGobbleRight{}{2}{1}{%
	\xs_StrLen{#1}[\xs_reserved_D]%
	\let\xs_reserved_E\relax
	\xs_exparg\xs_StrSplit_ii{\number\numexpr\xs_reserved_D-#2}{#1}%
	\xs_exparg\xs_assign_xstringresult{\xs_reserved_B}{#3}%
}

% renvoie #2 unités syntaxiques à la droite de la chaine #1
\xs_newmacro\StrRight{}{2}{1}{%
	\xs_StrLen{#1}[\xs_reserved_D]%
	\let\xs_reserved_E\relax
	\xs_exparg\xs_StrSplit_ii{\number\numexpr\xs_reserved_D-#2}{#1}%
	\xs_exparg\xs_assign_xstringresult{\xs_reserved_C}{#3}%
}

\xs_newmacro\StrChar{}{2}{1}{%
	\let\xs_reserved_B\empty\def\xs_reserved_C{#1}\def\xs_reserved_D{#2}%
	\ifnum#2>0
		\def\groupID{0}\def\xs_nestlevel{0}\integerpart0 \decimalpart0
		\let\xs_atbegingroup\relax
		\def\xs_atendofgroup{\expandafter\endgroup\expandafter\decimalpart\number\decimalpart\relax}%
		\def\xs_atnextsyntaxunit{%
			\ifnum\decimalpart=\xs_reserved_D% la n ième US est atteinte ?
				\edef\__temp{\def\noexpand\xs_reserved_B{\unexpanded\expandafter{\xs_reserved_A}}}% on capture l'US en cours qui est celle cherchée
				\expandafter\xs_exitallgroups\__temp
				\expandafter\xs_gobarg% stoppe la récursivité dans \xs_read_reserved_C
			\fi
		}%
		\xs_read_reserved_C
	\fi
	\xs_exparg\xs_ifempty{\xs_reserved_B}%
		{\gdef\groupID{}}
		{}%
	\xs_exparg\xs_assign_xstringresult{\xs_reserved_B}{#3}%
}

% Combien de fois compte t-on #2 dans #1 ?
\xs_newmacro\StrCount{}{2}{1}{%
	\def\xs_reserved_D{#1}\def\xs_reserved_E{#2}\let\xs_reserved_C\empty
	\xs_ifempty{#2}%
		{\xs_assign_xstringresult{0}{#3}%
		}
		{\decimalpart0 \integerpart0 \gdef\groupID{0}\def\xs_nestlevel{0}%
		\def\xs_atoccurfound{\let\xs_reserved_C\empty\xs_read_reserved_D}%
		\xs_read_reserved_D
		\xs_exparg\xs_assign_xstringresult{\number\decimalpart}{#3}%
		}%
}

% renvoie la position de l'occurrence #1 de la sous chaine #3 dans la chaine #2
\xs_newmacro\StrPosition{1}{2}{1}{%
	\xs_cutafteroccur{#2}{#3}{#1}%
	\let\xs_reserved_E\groupID
	\xs_ifx{\xs_reserved_C\xs_reserved_D}
		{\xs_assign_xstringresult{0}{#4}%
		\let\xs_reserved_E\empty
		}
		{\xs_exparg\xs_StrLen{\xs_reserved_C}[\xs_reserved_C]%
		\xs_exparg\xs_assign_xstringresult{\number\numexpr\xs_reserved_C+1}{#4}%
		}%
	\global\let\groupID\xs_reserved_E
}

\def\comparestrict{\def\xs_comparecoeff{1}}
\def\comparenormal{\def\xs_comparecoeff{0}}
\def\savecomparemode{\let\xs_saved_comparecoeff\xs_comparecoeff}
\def\restorecomparemode{\let\xs_comparecoeff\xs_saved_comparecoeff}

% Compare les deux arguments #1 et #2
% Renvoie 0 s'ils sont égaux et renvoie la
% position de la premiere unité syntaxiques différente sinon
\xs_newmacro*2\StrCompare{}{2}{1}{%
	\def\xs_reserved_A{#1}%
	\def\xs_reserved_B{#2}%
	\xs_ifx{\xs_reserved_B\xs_reserved_A}
		{\xs_assign_xstringresult{0}{#3}}
		{\xs_StrCompare_i{#1}{#2}{#3}}%
}

\long\def\xs_StrCompare_i#1#2#3{%
	\def\xs_StrCompare_iii##1{%
		\let\xs_reserved_A\empty
		\xs_exparg\xs_ifempty{\xs_reserved_C}%
			{\edef\xs_reserved_A{*\xs_comparecoeff}}%
			{\xs_exparg\xs_ifempty{\xs_reserved_D}%
				{\edef\xs_reserved_A{*\xs_comparecoeff}}
				{}%
			}%
		\def\xs_next{\xs_exparg\xs_assign_xstringresult{\number\numexpr##1\xs_reserved_A\relax}{#3}}%
	}%
	\def\xs_StrCompare_ii##1{% ##1 est la position
		\xs_exparg\xs_returnfirstsyntaxunit{\xs_reserved_C}\xs_reserved_A
		\xs_exparg\xs_returnfirstsyntaxunit{\xs_reserved_D}\xs_reserved_B
		\xs_ifx{\xs_reserved_B\xs_reserved_A}
			{\xs_exparg\xs_ifempty{\xs_reserved_A}%
				{\xs_StrCompare_iii{##1}% les 2 unités syntaxiques sont égales, on renvoie la position
				}
				{\def\xs_next{\xs_exparg\xs_StrCompare_ii{\number\numexpr##1+1}}% les 2 unités syntaxiques sont égales et non vides, on recommence
				\xs_exparg\xs_removefirstsyntaxunit{\xs_reserved_C}\xs_reserved_C
				\xs_exparg\xs_removefirstsyntaxunit{\xs_reserved_D}\xs_reserved_D
				}%
			}% les 2 unités syntaxiques sont différentes : on renvoie la position
			{\xs_StrCompare_iii{##1}%
			}%
		\xs_next
	}%
	\def\xs_reserved_C{#1}\def\xs_reserved_D{#2}%
	\xs_StrCompare_ii1%
}

\xs_newmacro\StrFindGroup{}{2}{1}{%
	\def\xs_reserved_A{#2}\def\xs_reserved_B{0}%
	\xs_ifx{\xs_reserved_A\xs_reserved_B}
		{\xs_assign_xstringresult{{#1}}{#3}}
		{\xs_StrFindGroup_i{#1}{#2}[#3]}%
}

\long\def\xs_StrFindGroup_i#1#2[#3]{%
	\def\xs_StrFindGroup_ii{%
		\xs_exparg\xs_ifempty{\xs_reserved_C}%
			{\xs_assign_xstringresult{}{#3}% s'il ne reste plus rien, on renvoie vide
			}
			{\xs_exparg\xs_returnfirstsyntaxunit{\xs_reserved_C}\xs_reserved_D
			\xs_ifx{\bgroup\xs_toks}% si la 1ère unité syntaxique est un groupe explicite
				{\advance\decimalpart1 % on augmente le compteur
				\xs_ifnum{\decimalpart=\xs_reserved_A\relax}% on est au groupe cherché lors de la profondeur courante ?
					{\xs_ifx{\empty\xs_reserved_B}% on est à la profondeur maximale ?
						{\xs_exparg\xs_assign_xstringresult{\xs_reserved_D}{#3}}% on renvoie ce groupe
						{\xs_exparg{\expandafter\xs_StrFindGroup_i\xs_reserved_D}{\xs_reserved_B}[#3]}% on recommence avec ce groupe et les profondeurs de recherche restantes
					}
					{\xs_exparg\xs_removefirstsyntaxunit{\xs_reserved_C}\xs_reserved_C
					\xs_StrFindGroup_ii
					}%
				}
				{\xs_exparg\xs_removefirstsyntaxunit{\xs_reserved_C}\xs_reserved_C
				\xs_StrFindGroup_ii
				}%
			}%
	}%
	\xs_extractgroupnumber{#2}\xs_reserved_A\xs_reserved_B
	\decimalpart0
	\xs_ifnum{\xs_reserved_A>0 }
		{\def\xs_reserved_C{#1}}
		{\let\xs_reserved_C\empty}%
	\xs_StrFindGroup_ii
}

\def\xs_extractgroupnumber#1#2#3{%
	\def\xs_extractgroupnumber_i##1,##2\_nil{\def#2{##1}\def#3{##2}}%
	\xs_extractgroupnumber_i#1,\_nil
	\ifx\empty#3\else\xs_extractgroupnumber_i#1\_nil\fi
}

\def\expandingroups{\let\xs_expandingroups\exploregroups}

\def\noexpandingroups{\let\xs_expandingroups\noexploregroups}

\def\StrExpand{\xs_testopt{\xs_StrExpand}{1}}
\long\def\xs_StrExpand[#1]#2#3{%
	\begingroup
		\xs_expandingroups
		\xs_ifnum{#1>0 }
			{\integerpart#1 \decimalpart0 \gdef\groupID{0}\def\xs_nestlevel{0}%
			\def\xs_atendofgroup{\xs_endgroup_eaddtomacro\xs_reserved_B{\expandafter{\xs_reserved_B}}}%
			\def\xs_atbegingroup{\let\xs_reserved_B\empty}%
			\def\xs_atnextsyntaxunit{\xs_eeaddtomacro\xs_reserved_B{\xs_reserved_A}}%
			\def\xs_reserved_C{#2}%
			\xs_StrExpand_i{#1}% Appel de la macro récursive
			}
			{\def\xs_reserved_B{#2}%
			}
		\expandafter
	\endgroup
	\expandafter\def\expandafter#3\expandafter{\xs_reserved_B}%
	\gdef\groupID{}%
}

\long\def\xs_StrExpand_i#1{%
	\xs_ifnum{#1>0 }
		{\let\xs_reserved_B\empty
		\xs_read_reserved_C
		\let\xs_reserved_C\xs_reserved_B
		\def\xs_reserved_A{\xs_exparg\xs_StrExpand_i{\number\numexpr#1-1}}%
		}
		{\let\xs_reserved_A\relax
		}%
	\xs_reserved_A
}

\def\scancs{\xs_testopt{\xs_scancs}{1}}
\long\def\xs_scancs[#1]#2#3{%
	\xs_StrExpand[#1]{#3}{#2}%
	\edef#2{\detokenize\expandafter{#2}}%
}

\restorexstringcatcode

\setverbdelim{|}%
\fullexpandarg\saveexpandmode
\comparenormal\savecomparemode
\noexploregroups\saveexploremode
\expandingroups

\endinput

                        H I S T O R I Q U E
------------------------------------------------------------------------------
v1.0    4/7/2008 : - Package achevé.
         7/7/2008 : - Package publié sur CTAN.
------------------------------------------------------------------------------
v1.1    15/8/2008
   - Le package ne nécessite plus LaTeX et est désormais utilisable sous
     Plain eTeX.
   - Ajout des macros \IfInteger et \IfDecimal.
     Pour cette dernière, la partie entière et la partie décimale sont
     récupérables dans les compteurs \integerpart et \decimalpart. Ce
     qu'il reste après qu'un caractère non attendu soit rencontré est
     dispo dans \xs_remainafterdecimal
   - Correction d'un bug dans \tokenize :
        suppression de l'expansion avec \normalexpandarg pour éviter le bug
        avec les lettres accentuées dans l'exemple : \tokenize\aa{éù}
   - Amélioration du code de la plupart des macros.
   - écriture d'une routine \xs_newmacro définissant les  macros.
   - Suppression de tous les compteurs grace à \numexpr.
   - Nouvelles fonctionnalités internes dans :
      \IfSubStr
        ajout des chaines se trouvant avant et après l'occurrence testée
        dans les sc \xs_behind_IfSubStr et \xs_before_IfSubStr
      \StrCount
        a) ajout de ce qui se trouve après la dernière occurrence dans la
           sc \xs_StrCount_afterlastocccur
        b) la macro ne dépend plus d'aucune autre
------------------------------------------------------------------------------
v1.2    23/8/2008
   - Amélioration du code de \StrMid \StrGobbleLeft, \StrLeft,
     \StrGobbleRight et \StrRight à l'aide de la nouvelle macro
     \xs_StrSplit_i
   - Nouveau test \IfStrEq qui compare 2 chaines
   - Nouveau test \IfEq qui compare 2 chaines (ou 2 nombres si les 2 chaines
     contiennent un nombre)
   - Correction d'un bug dans \xs_formatnumber. La macro n'envisageait pas le
     cas où son argument était vide ce qui faiasait planter
     \IfDecimal{}{V}{F} et \IfInteger{}{V}{F}
------------------------------------------------------------------------------
v1.3    21/9/2008
  - Amélioration du code, mise en place de récursivités terminales dans
    toutes les macros récursives, simplification de \xs_TestEqual en
    utilisant \ifx
  - Nouvelles macros \IfStrEqCase et \IfEqCase
      Teste si une chaîne est égale à plusieurs chaines données et
      exécute un code spécifique
  - Création de la macro publique \StrSplit
      Coupe la chaine en 2 à une position donnée
  - Nouvelle macro \StrCompare
      Compare 2 chaînes et renvoie la position du 1er caractère différent.
      Renvoie 0 si elles sont égales.
------------------------------------------------------------------------------
v1.3a   29/9/2008
  - Correction d'un bug : \expandafter#1
    dans les macros \IfSubStrBefore et \StrBetween qui buggue si #1 est un
    nombre > 9 !
  - Ré écriture de \xs_returnfirstsyntaxunit et \xs_gobarg qui
    deviennent purement développables.
  - Ré écriture de \StrLen
  - Nouvelle macro interne \xs_cutafteroccur
      Coupe la chaine après la nième occurrence d'une sous chaine.
  - Code amélioré de \StrMid, \StrLeft, \StrGobbleLeft, \StrRight,
    \StrGobbleRight grace à \xs_cutafteroccur
------------------------------------------------------------------------------
v1.4   4/11/2008
  - xstring traite ses arguments par unité syntaxique, et donc toutes les
    macros internes ont été ré-écrites à cette fin.
  - Le manuel a été ré-écrit, rendu plus clair et mieux structuré.
  - Nouvelle fonctionnalité : \expandarg
      le 1er lexème de chaque argument est 1-développé avant que la
      macro ne soit appelée. Si un argument comporte plus qu'1 lexème,
      il faut passer par \scancs*[1] pour 1-développer toutes les unités
      syntaxiques.
  - Correction de 2 erreurs dans le manuel anglais :  0 est la valeur par
    défaut dans \StrSubstitute et \StrDel
  - Cohérence dans les nom des séquences de contrôles temporaires qui
    sont désormais : \xs_reserved_A à \xs_reserved_E
------------------------------------------------------------------------------
v1.4a  12/11/2008
  - Correction d'un bug dans \xs_StrSplit dans le cas où l'argument
     numérique est <1 : la 1ere coupure doit être vide et le seconde doit
     être égale à l'argument.
------------------------------------------------------------------------------
v1.4b  16/11/2008
  - Correction de 2 bugs dans \xs_returnfirstsyntaxunit
------------------------------------------------------------------------------
v1.5   31/12/2008
  - Nouvelles fonctionnalités dans la recherche de groupes par un
    identificateur caractérisant leur imbrication. Implémentation de :
      1) \StrFindGroup
      2) \groupID
  - Ajout des nouvelles macros génériques \xs_read_reserved_C et
    \xs_read_reserved_D
  - Correction d'un bug dans \StrSplit : \StrSplit{{a}bc}{1}[\truc] faisait
    que \truc contenait «a{a}».
  - Correction d'un bug dans \xs_newmacro : l'argument optionnel était
    détokénisé à tort dans les macros étoilées.
  - Dans \xs_newmacro, on doit choisir le numéro du dernier argument devant
    être détokénisé dans le cas d'une macro étoilée (sachant que
     l'argument optionnel ne l'est jamais)
------------------------------------------------------------------------------
v1.5a  09/2/2009
  - Nouvelle macro \StrExpand, sensible au mode d'exploration. La macro est
    indépendante du mode d'exploration et dispose de ses propres commandes
    d'exploration : \expandingroups et \noexpandingroups
  - Ré-écriture de \scancs, qui devient triviale puisque dépendant de
    \StrExpand. Il n'y a plus de version étoilée et désormais, \scancs
    est sensible au mode d'exploration.
  - Correction d'un bug dans \IfInteger : \IfInteger{2.0}{V}{F} affichait F
  - Correction de bugs : mettre \let\xs_reserved_E\relax avant d'appeler
    \xs_StrSplit_i
  - Suppression des messages d'erreur, de warning et d'info. xstring devient
    donc silencieux ;)
  - Passage de 3 à 2 compteurs
  - Le manuel est désormais plus coloré, en espérant qu'il sera un peu
    plus agréable à lire !
------------------------------------------------------------------------------
v1.5b  13/3/2009
  - Modification d'un grand nombre de macros de telle sorte que vraiment
    n'importe quel code peut désormais être placé dans les arguments des
    macros (comme par exemple des \if, \ifx ou autre, même sans leur \fi, ce
    qui n'était pas possible jusqu'alors)
------------------------------------------------------------------------------
v1.5c  05/6/2009
  - Correction d'un bug dans \IfBeginWith : il faut appeler
    \xs_returnfirstsyntaxunit pour l'argument #2 puis pour l'argument #1 et
    non pas l'inverse pour que \xs_toks reflète ce qui se trouve dans #1
  - Correction d'un bug dans \xs_returnfirstsyntaxunit au cas où #1 commence
    par un espace : mettre \xs_toks à 0
  - Correction d'un bug dans \xs_returnfirstsyntaxunit :
    \xs_returnfirstsyntaxunit{{}}\truc
    faisait que \truc se développait en un espace.
  - Correction d'un bug dans \xs_removefirstsyntaxunit où le cas
    \xs_removefirstsyntaxunit{ {b}}\truc
    donnait \truc se développant en «b» au lieu de «{b}».
------------------------------------------------------------------------------
v1.5d  28/3/2010
  - Correction d'un bug dans \IfInteger : \afterinteger ne donnait pas le
    bon résultat. Par exemple avec 1.23 il renvoyait {} au lieu de {.23}
  - \xs_formatnumber ne detokenize plus ses arguments (que m'est-il passé
    par la tête pour que je code un truc comme ca ?), et donc
    \afterinteger et \xs_afterdecimal ont des tokens ayant le bon
    catcode
------------------------------------------------------------------------------
v1.6  24/10/2012
  - Correction d'un bug dans \xs_cutafteroccur au cas où #3<1
  - \IfDecimal ne \detokenize plus l'argument.
  - Nouvelle version de \tokenize qui enlevait les accolades si son argument
    était entre accolades
  - Nouvelle macro \StrCut
  - \xs_cutafteroccur_i ne produit plus d'espace indésirable si #3 était
    évalué par \numexpr
------------------------------------------------------------------------------
v1.7  13/1/2013
  - Correction d'un manque de rigueur dans les assignations concernant
    \groupID : elles sont toutes globales désormais
  - Les macros de xstring sont \long
------------------------------------------------------------------------------
v1.7a 28/2/2013
  - Correction d'un espace parasite dans \xs_removefirstsyntaxunit
------------------------------------------------------------------------------
v1.7b 29/7/2013
  - La date contenue dans \xstringdate est désormais conforme
------------------------------------------------------------------------------
v1.7c 13/10/2013
  - les macros impliquées dans \IfStrCase et \IfStrEqCase sont désormais \long
------------------------------------------------------------------------------
v1.8  07/12/2018
  - affectations globales supprimées (sauf pour \groupID) afin de ne pas
    surcharger la pile de sauvegarde
  - nettoyage du code, corrections de lourdeurs et maladresses
------------------------------------------------------------------------------
v1.81 09/12/2018
  - bug dans \IfInteger et \IfDecimal, la macro \xs_afterdecimal est indéfinie
    et doit être remplacée par \afterdecimal
------------------------------------------------------------------------------
v1.82 01/02/2019
  - \xs_testopt n'est pas longue et provoque un bug dans \xs_IfStrCase et
    \xs_IfStrCase lorsque #1 contient \par : \xs_testopt reste courte et
    \xs_IfStringCase a été modifiée pour que cela fonctionne.
    ------------------------------------------------------------------------------
v1.83 06/02/2019
      - mauvaise approche et mauvais fix dans la v1.82 : \xs_testopt devient
        longue, pas le choix (et donc aussi \xs_ifnxttok)
